Reducing Storage in Large-Scale Photo Sharing Services using Recompression

The popularity of photo sharing services has increased dramatically in recent years. Increases in users, quantity of photos, and quality/resolution of photos combined with the user expectation that photos are reliably stored indefinitely creates a growing burden on the storage backend of these services. We identify a new opportunity for storage savings with application-specific compression for photo sharing services: photo recompression. We explore new photo storage management techniques that are fast so they do not adversely affect photo download latency, are complementary to existing distributed erasure coding techniques, can efficiently be converted to the standard JPEG user devices expect, and significantly increase compression. We implement our photo recompression techniques in two novel codecs, ROMP and L-ROMP. ROMP is a lossless JPEG recompression codec that compresses typical photos 15% over standard JPEG. L-ROMP is a lossy JPEG recompression codec that distorts photos in a perceptually un-noticeable way and typically achieves 28% compression over standard JPEG. We estimate the benefits of our approach on Facebook's photo stack and find that our approaches can reduce the photo storage by 0.3-0.9x the logical size of the stored photos, and offer additional, collateral benefits to the photo caching stack, including 5-11% fewer requests to the backend storage, 15-31% reduction in wide-area bandwidth, and 16% reduction in external bandwidth.

==> algpseudocode.tex <==
\begin{algorithm}
\caption{My algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{MyProcedure}{}
\State $\textit{stringlen} \gets \text{length of }\textit{string}$
\State $i \gets \textit{patlen}$
\BState \emph{top}:
\If {$i > \textit{stringlen}$} \Return false
\EndIf
\State $j \gets \textit{patlen}$
\BState \emph{loop}:
\If {$\textit{string}(i) = \textit{path}(j)$}
\State $j \gets j-1$.
\State $i \gets i-1$.
\State \textbf{goto} \emph{loop}.
\State \textbf{close};
\EndIf
\State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
\State \textbf{goto} \emph{top}.
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> architecture.tex <==
\section{A New Image Compression Architecture}
\label{sec:architecture}
% Paper writing becomes much less formulaic after the introduction.
% Sometimes you will immediately go into the design of your system.
% Sometimes you will cover related work here instead of at the end.
% Sometimes you will give an intuitive tour of how your protocol/system
% works here before diving into details.  Most often you will provide a
% small amount of background and/or motivation so readers can fully
% grasp the problem you are solving and understand your contributions.

Compressing images from raw format can significantly reduce the image file size and meanwhile provide similar perceived image quality, and thus it is very popular to compress image before store or transfer it. Different image formats sit at different position of the compression ratio, encoding/decoding complexity tradeoff curve. In general, one can pay more encoding/decoding complexity for better compression ratio.

Depends on computational capability and storage scarcity, different users/devices may prefer different position of the complexity/compression tradeoff curve. JPEG serves most of the users/devices nicely, for its decent compression ratio and low encoding/decoding complexity. In traditional image compression architecture, where the sender wants to send an image to the receiver, if they both prefer JPEG compression, sender will just encode the image to JPEG format and send the JPEG representation of the image to the receiver; the receiver then decode the JPEG to view the image.

However, there are some other users/devices prefer a different position of tradeoff curve other than JPEG sits at, for example, Facebook. Facebook has to store tons of images and even a small reduction on image file size can significantly reduce its operational cost. In addition, Facebook's computational capability can afford some extra complexity. As a result, Facebook is willing to pay a bit extra complexity, to get better compression ratio.

We propose a new image compression architecture for this image sharing sites and their users' scenario, where image sharing sites (Facebook) can change the image format, only internally, to further compress the image. Such ``re-formatting opportunity'' does not exist in traditional sender/receiver image compression architecture because both sender and receiver possess similar computational capability as well as storage scarcity and thus they prefer the same image format. The challenge is to design such compression to offer both good compression gain and acceptable low complexity at the same time.

==> background.tex <==
\section{JPEG and Its Entropy Coder}
\label{sec:background}

The JPEG (Joint Photographic Experts Group) image representation
format is widely used by photo sharing services. JPEG compresses
images using multiple steps. In this section, we describe these steps.
% with special emphasis on
% %one of the
% %steps, 
% \emph{entropy coding}: \sysname replaces the standard entropy
% coder with one that leverages the 
% %AO I think it's the scale, and not the architecture, that plays a primary role in enabling the methods we proposed
% %architecture 
% scale 
% of modern photo sharing
% services.%  to achieve greater compression gain than previously possible
% without significantly increasing the complexity of compression. 

% \ao{I think this has to be more nuanced, i.e., one can achieve more compression already (e.g., HEVC), so it has to be more than previously possible, while preserving compatibility with JPEG in some sense. But we also need to keep in mind the PackJPEG software. We could make the point that we achieve greater compression with very high speed (unlike other schemes) thanks to our aggressive use of memory. }

%, its degree of compression can be adjusted, allowing a selectable tradeoff between compressed image size and image quality 

% \begin{figure}
% \centering
% \begin{minipage}[t]{0.5\textwidth}  \epsfig{file=pics/jpeg_encoding.eps,  width=\linewidth}
%   \caption{JPEG Encoding Steps}
%  \label{fig:jpeg_encoding}
% \end{minipage}
% \end{figure}

% \subsection{JPEG Encoding Steps}

\parab{Overview and Principles.} JPEG is a block-based coder: it
independently transforms each \emph{block} of 8x8 pixels in the entire
image, and outputs, for each block, a compressed bitstream. Operating
at the granularity of a block represents a tradeoff between the
computational complexity of compression and the degree of correlation
one can exploit within neighboring pixels. For each block, JPEG first
does an initial color space conversion: this represents a coordinate
transformation from an RGB representation to one that separately
captures color (chrominance) and brightness (luminance), and has been
shown to improve compressibility.  

Each block then undergoes three distinct steps~\cite{jpeg_still}:
pixel to frequency domain conversion, which leverages the observation
that natural images are \emph{sparse} in the frequency domain (i.e.,
that most of the ``energy'' in the image is concentrated in a few
frequencies), thereby enhancing compressibility; quantization, a lossy
step that discards visually insignificant information; and entropy
coding, which exploits the sparsity and the statistics of images to
losslessly compress the 
quantized 
frequency domain representation. The following
paragraphs describe these three steps. We omit a description of image
decompression, which performs the inverse of each step in the reverse
order. 

% Figure~\ref{fig:jpeg_encoding} illustrates important encoding steps of JPEG. For a given image, each of its color component will be divided into multiple 8x8 blocks. Those blocks are independent inputs, go through encoding steps sequentially, and output as compressed data stream. At a high level, %the 8x8 blocks will be first shifted from unsigned integers to signed integers, then % in \emph{DCT step}, Forward DCT (FDCT) transforms each 8x8 block to 64 \emph{DCT coefficients}. Those DCT coefficients are then quantized by a 64-element quantization table in \emph{quantization step}, to discard unnecessary information that is not visually important \cite{jpeg_still}. The final encoding step is \emph{entropy encoding} , which losslessly compresses quantized DCT coefficients, by leveraging their statistical characteristics.

\parab{Frequency Domain Conversion.} JPEG transforms each 8x8 block of
pixels into the frequency domain using the Forward Discrete Cosine
Transform (F-DCT). The output of this step is a set of 64
\emph{coefficients}; each coefficient represents the amplitude of a
specific frequency (DCT defines a set of 64 orthogonal
frequencies). Intuitively, the amplitude is a measure of the
``energy'' associated with the corresponding frequency.  In 8x8 blocks
of natural images, it has been observed that only a few (usually a
handful) of the 64 frequencies have non-trivial associated energy, a
property that enhances compressibility. The coefficient associated
with the zero frequency is called the \emph{DC coefficient}, and the
other 63 coefficients are called \emph{AC coefficients}. 

% which represents 64 discrete signal in spatial domain (pixel % domain). FDCT transforms such spatial domain signal to 64 orthogonal % frequencies, i.e., frequency domain, and outputs 64 basis-signal % amplitudes, so called DCT coefficients. The coefficient of zero % frequency is called the \emph{DC coefficient}; other 63 coefficients % are called \emph{AC coefficients}.

% rephrasing from jpegstill paper: % Each 8x8 block of source image samples is effectively a 64-point discrete signal which is a % function of the two spatial dimensions x and y. The % FDCT takes such a signal as its input and decomposes % it into 64 orthogonal basis signals. Each contains one % of the 64 unique two-dimensional (2D) “spatial % frequencies’’ which comprise the input signal’s % “spectrum.” The ouput of the FDCT is the set of 64 % basis-signal amplitudes or “DCT coefficients” whose % values are uniquely determined by the particular % 64-point input signal. % The DCT coefficient values can thus be regarded as the % relative amount of the 2D spatial frequencies contained % in the 64-point input signal. The coefficient with zero % frequency in both dimensions is called the “DC % coefficient” and the remaining 63 coefficients are % called the “AC coefficients.’’ 

\parab{Quantization.} In this step, each coefficient is divided by a
number corresponding to the \emph{quantization step size} and then
rounded to the nearest integer, which effectively discards some of the
least significant bits (i.e., reduces the precision) in each
coefficient.  A smaller quantization step size reduces precision by a
smaller amount. In general, JPEG uses smaller quantization step sizes
for lower frequencies, because human vision is known to be
frequency-sensitive and can perceive distortion 
more easily at lower frequencies
than at higher. The collection of quantization step sizes forms a
\emph{quantization table}\footnote{JPEG actually has two tables: one
  for chrominance and the other for luminance: we have simplified the
  description for explanatory purposes.}.  Finally, users can adjust 
the degree of quantization by specifying a \emph{quality parameter} or QP (a
number between 1 and 100): JPEG uses this to scale further the quantization
step size: a larger quality parameter represents less loss
of precision (the quantization step size is essentially divided by QP, so that a larger QP leads to a smaller resulting step size and thus better quality). 

% and these quantizers together form a % \emph{quantization table}. The choice of quantizers controls the % precision and quality of the image % precision and thus the quality of the image. For example, human eyes % are more sensitive to low frequency signals, so in general JPEG % chooses smaller quantizers for low frequency as comparing to high % frequency ones.

% JPEG standard defines two default quantization tables (one for luminance and one for chrominance). By modifying default quantization table, JPEG can choose the tradeoff between compressed image size and image quality, and output images with different \emph{quality parameter}. For a desired quality parameter, JPEG modifies the quantization table by applying the same scaling calculation on all the quantizers. For example, the quantization table for a high quality parameter needs to divide each default quantizer by a large number, leads to a small quantizer which preserves better precision in the quantization step.

% repharsing from jpegstill paper: % Each element can be any integer value from 1 % to 255, which specifies the step size of the quantizer for % its corresponding DCT coefficient. The purpose of % quantization is to achieve further compression by % representing DCT coefficients with no greater precision % than is necessary to achieve the desired image quality. % Stated another way, the goal of this processing step is % to discard information which is not visually significant. % Quantization is a many-to-one mapping, and therefore % is fundamentally lossy. It is the principal source of % lossiness in DCT-based encoders. % Quantization is defined as division of each DCT % coefficient by its corresponding quantizer step size, % followed by rounding to the nearest integer:

% When the aim is to compress the image as much as % possible without visible artifacts, each step size ideally % should be chosen as the perceptual threshold or “just % noticeable difference” for the visual contribution of its % corresponding cosine basis function. These thresholds % are also functions of the source image characteristics, % display characteristics and viewing distance. For % applications in which these variables can be reasonably % well defined, psychovisual experiments can be % performed to determine the best thresholds. The % experiment described in [12] has led to a set of % Quantization Tables for CCIR-601 [4] images and % displays. These have been used experimentally by % JPEG members and will appear in the ISO standard as a % matter of information, but not as a requirement.

% JPEG's entropy coder arranges the quantized DCT coefficients as a list of integer values\footnote{The DCT coefficients of an 8x8 pixel block are also arranged as an 8x8 matrix. Before entropy coding, JPEG uses a \emph{zigzag} scan on this matrix, which results in a 64-element sequence of coefficients, with lower frequency coefficients generally appearing earlier in the sequence than higher frequence coefficients.} and generates a compressed data stream. \sysname replaces JPEG's standard entropy coder with a more sophisticated one. JPEG specifies two entropy coding methods, Huffman coding~\cite{huffman} and arithmetic coding~\cite{arithmetic}, and \sysname's uses Huffman coding, which we now describe.

% \begin{table} \centering \begin{tabular}{ c c } \textbf{symbol-1} & \textbf{symbol-2} \\  (RUNLENGTH, SIZE) & (AMPLITUDE) \\ \end{tabular} \caption{Intermediate Symbols for AC coefficients} \label{tbl:inter_symbols} \end{table}

\parab{Entropy Coding.} JPEG's entropy coder compresses the quantized coefficients using three key ideas\footnote{Our simplified description omits some details: we refer interested readers to~\cite{jpeg_still}}.

%\ao{I included back a reference to zig-zag scanning, which is an important part of the entropy coding.}
First, because natural images are often predominantly smooth, low DCT
frequencies are much more likely to have large values than high
frequencies. Thus, JPEG first uses a \emph{zigzag} scan to re-arrange
those 2 dimensional 8x8 DCT coefficients into a 1 dimensional array of
64 coefficients. This zigzag sequence approximately orders DCT
coefficients from low frequency to high frequency.  This enables a
special \emph{End-of-Block} (EOB) code, which is used to signal that
the remaining coefficients along the zigzag scan are all
zero-valued. The zigzag order is chosen so that, on average, the EOB
comes at quickly as possible (i.e., coefficients likely to be large
are scanned first) leading to significant compression.

Second, because of sparsity, most coefficients within a block are
zero-valued, so run-length encoding (by which a sequence of
consecutive zeros is represented by the length of the sequence) can
significantly compress the coefficients. Specifically, consider a
sequence of $k$ zero-valued coefficients, followed by a non-zero
coefficient whose value is $c$. JPEG represents these by two
quantities: \syma and \symb. \symb represents the value $c$, but \syma
represents two components $(k,l)$ where $l$ is the smallest number of
bits required to represent $c$, based on a table that assigns
increasing sizes to larger coefficients ($1$ bit is needed to
represent $+1$ and $-1$, $2$ bits 
to represent $-3,-2,2,3$, $3$ bits to
represent $-7, -6, -5, -4, 4, 5, 6, 7$ and so on.). 
%\ao{Added an explanation below. If this is too obvious, it can be removed.}
% This is a simple application of the fundamental information theoretic 
% result that for optimal compression one assigns shorter codes (using fewer bits) to the most likely events (in this case
% the smaller coefficients). 

%(i.e., the \emph{run}-length and the %\emph{size}).  Thus, for example, the sequence of quantized coefficients $[0,5,0,0,0,3 \cdots]$ is represented by two \syma tuples: $<1,3>$ and $<3,2>$. Finally, JPEG defines a special \emph{End-of-Block} value for \syma, which specifies that the remaining coefficients (recall that there are, in total, 64 coefficients) are all zero-valued.

% \ao{I added some text above to clarify "minimum number of bits to represent a coefficient. In the end this is really a Huffman table for the size, it's just that it's separated into the size term and the amplitude.}

Third, instead of representing each \syma directly, it replaces each
distinct \syma with a Huffman code. The intuition is that more likely
\syma values should be represented using codes with fewer bits. This
step is achieved using a \emph{Huffman
  table}. Table~\ref{tbl:table_comparison} shows a snippet of JPEG's
default Huffman table. In this table, the \syma $(0,1)$ and $(0,2)$
occur most frequently, so they can each be represented using a unique
2 bit code (e.g., 00 and 01). Other \symas are assigned longer codes,
since they are expected to occur less frequently.  More precisely,
JPEG uses 4 separate Huffman tables, for chrominance, luminance, the
DC coefficient and the AC coefficients.

% Note that JPEG defines standard tables, but a JPEG implementation can
% also choose to generate per-image tables that can be attached to the
% file header in order to improve compressibility by matching better the
% specific image statistics, at the cost of some increase in complexity.
% However, this approach may not be efficient if the rate required to
% transmit these custom tables is greater than the savings achieved by
% better matching image statistics.  % Our proposed methods, to be
% described next, can be viewed as creating more complex and specialized
% tables, but essentially "spreading" their rate overhead across all
% stored images.  Further, these tables result in no communication
% overhead, since stored images are converted to standard JPEG before
% being sent to end users.

% JPEG Huffman coding is a 2-step process. The first step converts the quantized coefficients into intermediate symbols. The second step converts the symbols to data stream. % % below rephrased from jpeg-still paper % In the first step, JPEG first uses \emph{zigzag} sequence to arrange those 2 dimensional 8x8 DCT coefficients to a 1 dimensional array of 64 coefficients. This zigzag sequence generally orders DCT coefficients from low frequency to high frequency. The DC coefficient is the first one in this array, followed by 63 AC coefficients. Below we first describe how does JPEG encode AC coefficients, followed by encoding DC coefficients, which is just a simpler variant.

% Each nonzero AC coefficient, plus the zero coefficients that precede it in the zigzag sequence, are represented in a pair of symbols, \emph{symbol-1} and \emph{symbol-2}, shown in Table~\ref{tbl:inter_symbols}. Symbol-1 contains two pieces of information, RUNLENGTH\footnote{For the rest of the paper, we call it RUN for short.}, the number of consecutive zero coefficients preceding the nonzero coefficient; and SIZE, the number of bits needed to represent the nonzero coefficient, where: % \begin{equation} % SIZE=\left\lfloor{\log_2{AMPLITUDE}}\right \rfloor + 1 % \label{formula:amplitude_to_size} % \end{equation}

% Symbol-2 contains single piece of information, which is the AMPLITUDE of the nonzero AC coefficient, contains SIZE bits as signaled in symbol-1. For example, quantized coefficients $[0,5,0,0,0,3 \cdots]$ contains two nonzero coefficients and thus are represented as two pairs of symbols. First symbol-1 is (RUN 1, SIZE 3) and second symbol-1 is (RUN 3, SIZE 2). In addition, there is a special symbol-1, the \emph{End Of Block} (EOB), which indicates that all following DCT coefficients are 0 in this block and thus it is the end of encoding this block. \xx{actually, there is another special symbol-1, representing 16 consecutive 0s. but to explain that we have to explain RUN is upperbounded by 15, not sure if we should go into that detail.}

% The second step takes above intermediate symbols, uses variable-length code to represent symbol-1s. To minimize the number of bits needed to represent all the symbol-1s, intuitively, frequently occurred symbol-1s should be represented by a shorter code compared to rarely occurred ones. JPEG's entropy coder achieves this by calculating the statistical characteristics of symbol-1 to get an optimized Huffman table. JPEG standard Huffman table is partially shown in the left column of Table~\ref{tbl:table_comparison}. % % above rephrased from jpeg-still paper

% The intermediate symbols for encoding DC coefficients is similar to Table~\ref{tbl:inter_symbols}, the only difference is that its symbol-1 only contains the SIZE information. Instead of encoding the DC coefficient as AMPLITUDE directly, JPEG encodes the difference between current DC coefficient and the DC coefficient of previous block, because DC coefficients of nearby blocks are similar, usually the AMPLITUDE of difference needs less bits than the AMPLITUDE of original DC coefficient.%JPEG uses such difference as AMPLITUDE and calculates the SIZE according to Formula~\ref{formula:amplitude_to_size}. % JPEG uses a different Huffman table for symbol-1s of DC coefficients.

% Each JPEG file attaches 4 Huffman tables in the file header: for both luminance and chrominance components, there is a Huffman table for AC coefficients and a Huffman table for DC coefficients. Each JPEG file can choose to use the default Huffman tables, i.e., JPEG standard file, or choose to optimize those 4 Huffman tables for current input image, i.e., JPEG optimize file. \sysname optimizes those Huffman tables in a different way to offer better compression.


==> codec.tex <==
\section{A Context Sensitive Lossless Coder}
\label{sec:codec}

% comments from Ramesh
% sec 2: reduce storage, our approach is only good if we save more machinges for saving (we also need to buy new machines for encoding/decoding)
% sec 3.1: more background on JPEG (other parts otherthan the entropy part)
% demonstrate how different huffman table can be, add JPEG std/opt to table 1, move it to 3.2, intuition of the scheme and the overview of the approach (restructure 3.2)
% 3.2.2, after formula, i should explain training/testing before "whereSIZE()calculates  the  bits  of  the  coefficient,maxSIZE(i)is   observed   maximum   coefficient   SIZE   
% forzigzag positioni." across training images, i should explain the trainig/testing in overview

% 3.2.3 formular two, change to SIZE(b_i(j))

% 3.3 training procedure is not optimized

% overview in 3.2, intuition for context sensing, smoothing 

% describe why i get 1%

\begin{table}
\small
\centering
\begin{tabular}{@{}*6c@{}}
\toprule[1.5pt]
\multicolumn{2}{c}{\textbf{JPEG Standard}} & \multicolumn{2}{c}{\textbf{Context}$<5,0,0>$} & \multicolumn{2}{c}{\textbf{Context}$<2,5,9>$} \\
\textit{Bits} & \emph{runsize} & \textit{Bits} & \emph{runsize} & \textit{Bits} & \emph{runsize} \\ 
\cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
2 & (0, 1) &1 & EOB & 2 & (0,4) \\
2 & (0, 2) &2 & (0, 1) & 2 & (0,5)\\
3 & (0, 3) &4 & (2, 1) & 3 & (0,2)\\
4 & EOB    &4 & (1, 1) & 3 & (0,3)\\
%4 & (0, 4) &3 & (0, 6) & 4 & (4, 1) \\
%4 & (1, 1) &4 & (0, 1) & 6 & (0, 2) \\
%5 & (0, 5) &6 & (0, 7) & 6 & (1, 1) \\
%5 & (1, 2) &7 & (1, 1) & 7 & (7, 1) \\
%5 & (2, 1) &7 & (1, 2) & 8 & (5, 1) \\
%6 & (3, 1) &7 & (1, 3) & 8 & (6, 1) \\
%6 & (4, 1) &7 & (1, 4) & 9 & (0, 3) \\
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
7 & (0, 6) &9 & (0, 5)    & 9 & EOB \\
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
\bottomrule[1.5pt]
\end{tabular}
\caption{JPEG Standard Huffman Table vs. Huffman Tables of 2 Contexts of \sysname. Context $<5,0,0>$ is used to encodes \symas at position 5, with 0 index for both intra- and inter-block energy, i.e., smallest energy; it is expecting more zero-valued coefficients, and thus we can see it only uses 1 bit for EOB, and also less bits for 1 bit amplitude. In contrast, Context $<2,5,9>$ expects more energy, as it uses less bits for large amplitudes without zero-valued coefficients before them, and 9 bits for EOB.}
\label{tbl:table_comparison}
\end{table}

\begin{figure}[t]
%  \centering\epsfig{file=../pics/sysname.eps,  width=0.65\linewidth}
  \includegraphics[width=0.65\linewidth]{../pics/sysname}
  \caption{\sysname Encoding Architecture}
 \label{fig:sysname}
\end{figure}

In this section, we describe the core of \sysname, a new entropy coder
that provides significant compression gains over JPEG without
significantly increasing image processing complexity.  We begin with
an overview of our approach, then discuss the details of our design.

\subsection{The Approach}

\parab{Design constraints.} In any compression algorithm, there is a
tradeoff between the \emph{complexity} (the computational cost) of
compression/decompression and the \emph{compression gain}
achieved. For photo-sharing services, it is essential to design a low
complexity codec since decoding delays can adversely affect user
experience.

A related, but subtly different, consideration is
\emph{JPEG-compatibility}. The vast majority of photos uploaded to
photo sharing services are in the JPEG format, as this is the dominant
compressed format produced by the digital cameras, smart phones and
tablets with which these shared photos are initially taken.  There
exist other image compression and decompression
algorithms~\cite{jpeg2000,webp} %\rg{Add ref to webp, jpeg2000}
that achieve better compression at the same quality, but to use these
would require converting an uploaded JPEG image into the pixel domain,
and then applying the corresponding compression algorithm, which can
add complexity.
% . Not only
% can this approach add complexity, it can also negate the robustness
% benefits of JPEG: the standard is mature and understood well-enough to
% be applied at the scale of modern photo sharing services, and moving
% away from this might incur significant development and infrastructure
% investments. \rg{AO, please check.} \ao{RG: I think this is a fair
%   point, although once most of decoding is software-based it should
%   not be that difficult to change, e.g., using webp for the final
%   delivery to the user. I think the predominant factor is that all
%   hardware acquisition, phones, cameras, etc are JPEG, and so changing
%   the storage would require doing extra work for almost all incoming
%   images. }

So, \sysname takes a pragmatic position in the design space: it
re-uses most of the JPEG processing steps, and only changes its
entropy coder. This has a desirable property: when a JPEG image is
uploaded, \sysname does not need to convert the image to the pixel
domain. Instead, it reverses the default entropy coding step in the
uploaded image, and re-codes the resulting quantized coefficients
using the new entropy coder. As a result, \sysname can be
incrementally deployed at various locations in the photo stack of
large-scale photo sharing services (Section~\ref{sec:integrating}).

However, in a dramatic departure from JPEG, \sysname exploits a degree
of freedom enabled by its intended use within the confines of a photo
sharing service. JPEG is engineered to minimize its coding (e.g., its
quantization and Huffman) tables. Because any custom made Huffman
tables would have to be transmitted to the receiver, and this would
incur storage and transmission overhead, most shared JPEG images use
default tables that are small and were originally designed based on
\emph{average} statistics of \emph{typical} images.  \sysname, because
it is designed to be used within a photo sharing service, can use
large coding tables (which can capture more fine grained statistical
dependencies).  As long as these tables are small enough to be cached
in memory, \sysname can efficiently compress or decompress
images. Using this idea, as we quantify in Section~\ref{sec:eval},
\sysname achieves enough compression gains to justify, we believe,
incorporating into large-scale photo sharing services; at the scale of
these services, even gains in the 15-30\% range can be significant.

% RG: I removed this footnote, not clear the audience will appreciate it
% \footnote{Note that these significantly larger tables could be
%   used as ``default'' tables, thus incurring no additional
%   communications overhead, but accommodating tables of this size would
%   have been completely impractical in the technology context of the
%   early 90s when JPEG was being finalized.}.

% The downside of our pragmatic approach is that one expects lower
% compression gains than those available by using a completely new
% compression algorithm. JPEG already eliminates significant redundancy
% in images, so minimal changes to its processing steps might only yield
% diminishing returns. Despite this, 

% \ao{I changed the range to 15-30\% since this is what we achieve with \lossyname}
% \rg{We need a nice figure to represent the key ideas.}

\parab{Context-Sensitive Coding.} \sysname exploits the freedom to
have large coding tables by designing \emph{context-sensitive coding
  tables} that result in lossless\footnote{Lossless with respect to
  the uploaded JPEG image.} compression. Recall that JPEG's Huffman
tables are used to code \symas, based on the expected frequency of
occurrence of \symas in the block. \sysname \emph{learns}
context-sensitive Huffman tables by learning the empirical probability
of occurrence of \symas from a corpus of images. This learning
leverages the availability of such corpora in a large-scale photo
service.

But what do we mean by \emph{context-sensitivity}? \sysname uses two
insights derived from properties of natural images. To understand the
first insight, recall that JPEG linearizes the coefficients using a
zigzag scan. We use the term \emph{position} to denote the index of a
given coefficient in the array.

% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}{0.33\textwidth}
%     \epsfig{file=../pics/position_distribution.eps,  width=\linewidth}
%     \caption{Probabilities of 3 Bit Coefficients}
%     \label{fig:position_distribution}
%   \end{subfigure}
%   \begin{subfigure}{0.33\textwidth}
%     \epsfig{file=../pics/position_symbol_distribution.eps,  width=\linewidth}
%     \caption{Probabilities of Symbol-1 (0, 3)}
%     \label{fig:position_symbol_distribution}
%   \end{subfigure}
%   \begin{subfigure}{0.33\textwidth}
%     \epsfig{file=../pics/position_0_distribution.eps,  width=\linewidth}
%     \caption{Probabilities of Symbol-1 End-of-Block}
%     \label{fig:position_0_distribution}
%   \end{subfigure}
%   \caption{Probabilites of different coefficients and symbols change
%     with zigzag position.  This insight allows the contexts in
%     \sysname to encode them with fewer bits.}
% \end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{../exps/scatter/scatter_prob_zigzag2.pdf}
    \caption{Probabilities of 3 Bit Coefficients as a function of position.}
    \label{fig:position_distribution}
\end{figure}

\parab{Position-dependence.}
The first insight \sysname uses is that the empirical probability of
occurrence of a \syma can depend upon its position. A \syma
corresponds to a run of zero-valued coefficients, followed by a
non-zero coefficient $x$ occurring at position $p$. 

% \ao{Not a big deal, but we are using $x$ for position, where before $x$ was used for the coefficient value. Maybe the easiest would be to change the term we use for the coefficient in the previous section.}
%\xx{done, change previous 'x' to 'c'.}

Consider the same \syma $(k,l)$ occurring at two different positions
$p_a$ and $p_b$.  The key observation we make is: the empirical
probability of occurrence of $(k,l)$ at $p_a$ is likely to be very
different from that at $p_b$ (Figure~\ref{fig:position_distribution}
illustrates this). This follows from the fact that, for natural
images, it is known that non-zero coefficients are increasingly
unlikely at higher frequencies~\cite{lam2000DCT}.
%
%(in fact, exponentially~\cite{laplacian}) 
%unlikely at higher frequencies. 
For this reason, \sysname generates different tables for different
positions: i.e., position is one aspect of the context used for
encoding.

\begin{figure}[t]
\centering
%  \epsfig{file=../pics/unnatural_block.eps,  width=0.7\linewidth}
  \includegraphics[width=0.7\linewidth]{../pics/unnatural_block.eps}

  \caption{Natural and Synthetic Blocks}
 \label{fig:unnatural_block}
\end{figure}

% As an example, Figure~\ref{fig:position_distribution} plots the
% probability of appearance of coefficients of size 3 (i.e., requiring 3
% bits) at different positions \footnote{
% \ao{Is there any reference for where this image set can be found?} The probabilities are derived
%   from a hundred 600x600 images with quality factor 75. We use the
%   same image set for other plots by default.}. Coefficients of this
% size occur frequently at positions 2-10, but rarely after position 20.
% This shows that the probabilities of \symas of size 3 are
% position-dependent.  As another example,
% Figure~\ref{fig:position_symbol_distribution} illustrates the
% position-dependence of \syma $(0,3)$. 
% %
% \xx{we may want to put
%   Figure~\ref{fig:position_distribution} and
%   Figure~\ref{fig:position_symbol_distribution} together.} 
%   %
% Similarly, as Figure~\ref{fig:position_0_distribution} shows, the
% End-of-Block (EOB) symbol occurs more frequently at higher frequencies.

%\ao{rewrote the beginning of this paragraph}

\parab{Energy-dependence.}
The second insight is based on the observation that, relative to image
sizes predominantly in use today, an $8\times 8$ block represents a
very small patch of the image.  To see this, imagine capturing the
same visual information (a photo of a person, say) with two cameras of
different resolutions, and then use JPEG encoding for both
images. Clearly $8 \times 8$ blocks in the higher resolution image
represent smaller regions of the field of view, and thus will tend to
be smoother.  This has two useful implications. First, information
within a block will tend to be smooth, with additional smoothness
expected for larger images. Smoother images are such that coefficients
at higher frequencies tend to be smaller. Second, because the same
region in the field of view comprises more blocks when larger images
(higher resolutions) are generated, it becomes more likely that
neighboring blocks will have similar characteristics.

%Because natural images are smooth (they do not
%have significant discontinuities, unlike synthetically generated
%images, like, for example Moir\'{e} patterns), 

We exploit these two ideas by creating tables such that the
probability of occurrence of a \syma at a given position can also
depend upon
%the
%actual \symbs of coefficients both within a block, and in neighboring
%blocks.
%More specifically, the likelihood of a given \syma can also depend
%upon 
the \emph{energy} of other coefficients with within the block
(\emph{intra-block} energy) and of neighboring blocks
(\emph{inter-block} energy), where \emph{energy} of a set of
coefficients is computed as the sum of squares of the \symb of those
coefficients.

%The square of the \symb of a coefficient is termed the \emph{energy}
%of a coefficient. 
%
To illustrate the role of \emph{intra-block} energy
Figure~\ref{fig:unnatural_block} (a) depicts a block from a real world
image, together with the linearized coefficients, while
Figure~\ref{fig:unnatural_block} (b) depicts a synthetically generated
block.
%
Notice that the \emph{energy} (the square of the amplitudes) of the
coefficients decays smoothly with frequency in the natural image
block, but the synthetic block does not exhibit such behavior.  Thus,
when encoding a specific \syma at a given position within a block, if
the total energy of the coefficients transmitted before that position
was relatively small, then the likelihood of \syma corresponding to a
large coefficient will also be small.

By contrast, JPEG assumes that for {\em any} coefficient, smaller
values are more likely. Position-dependent coding assumes that it is
more likely that smaller coefficients will be encountered at higher
frequencies (independent of other coefficients in the block). This
energy-dependent context is based on the assumption that observed
energies in previously encoded coefficients can further help
characterize the statistics of coefficients to be encoded.

%This decay in \emph{intra-block} energy
%dictates the likelihood of specific amplitudes at a given position
%within a given block, and, by extension, the likelihood of a specific
% (since the \syma encodes the number of bits
%required to express the amplitude). 

Finally, since neighboring blocks are likely to be similar, especially
at high resolutions, the probability of a \syma at a given position
within a given block can also depend upon the energy of the
immediately neighboring blocks.

For this reason, \syma uses \emph{intra-block} energy and
\emph{inter-block} energy as additional pieces of context.

\parab{Putting it all together.}
Thus, context in \sysname is defined by a triple: position,
intra-block energy, and inter-block energy. At a high-level, \sysname
works as follows (Figure~\ref{fig:sysname}):
\begin{itemize}[leftmargin=*]
\item From a training set of images, \sysname learns a Huffman table
  for each unique context (i.e., for each unique combination of
  position, intra- and inter-block energy). In practice, there are
  100s of unique contexts.
\item When an image is uploaded, \sysname reverses the entropy code in
  the incoming image, then uses the learned Huffman tables to re-code
  the image.
\item Before delivering an image to a client, \sysname reverses its
  context-sensitive entropy code, then applies the default JPEG
  entropy code. A photo-sharing service may apply other
  transformations (resizing, or transcoding to another format) after
  this step.
\end{itemize}
%The following subsections describe some of these details.

% \ao{symbol-1s probably refers to \syma? Also, if we are going to be talking about SIZE 3, SIZE 4, etc this should be consistent with the notation in the previous section, so the notation can be introduced in the previous section. }
% We propose a context sensitive entropy coder to replace JPEG's in Figure~\ref{fig:jpeg_encoding} to encode symbol-1s more efficiently. Instead of using one single Huffman table as the JPEG standard and JPEG optimized do, we achieve better compression by separating symbol-1s into different \textit{contexts} and using different Huffman tables for different contexts. If different contexts have different statistical characteristics of symbol-1s, then it indicates that symbol-1s can be encoded more efficiently using multiple Huffman tables than using a single Huffman table. In Table~\ref{tbl:table_comparison}, we list and compare the least bits symbol-1s (the most frequently occurring symbol-1s) of Huffman table of JPEG standard and Huffman tables of two different contexts of \sysname. Both contexts' Huffman tables are quite different to JPEG standard Huffman table. Context A is used to represent larger coefficients, as it uses less bits for symbol-1s of 0 RUN but larger SIZE, e.g., 2 bits for (0, 5) which is 5 bits in JPEG standard Huffman table; also it uses 9 bits for end-of-block (EOB), which is 4 bits in JPEG standard table, showing that the block is very unlikely to end in this context. On the other hand, context B favors smaller coefficients, it uses only 1 bit for EOB meaning that the block will be ended with high probability.

% Better compression comes from using different Huffman table to encode symbol-1s. The challenge is how to define contexts such that the statistical characteristics of symbol-1s of different contexts are different, i.e., so that using different Huffman tables offers better encoding efficiency. Note that JPEG allows image-specific  Huffman tables to be included in the file header. We do not follow this approach because our Huffman tables are not compatible with JPEG and also because their size is so large that adding them to individual images would prevent compression gains from being achieved. Thus, the Huffman tables of \sysname need to be designed to optimize average behavior across a broad class of images. 
% %so that context to capture the common information across images, but not the biased information for a particular image. 
% To tackle these challeges, we use three properties to define context, the zigzag position of current symbol-1 (Section~\ref{sec:zigzag_position}), the intra block energy value (Section~\ref{sec:intra_value}) and the inter block energy value (Section~\ref{sec:inter_value}). The intuitions behind choosing these three properties are as follows: 1) JPEG quantization step makes coefficients at different zigzag positions follow different distributions, which leads to different Huffman tables if we separate symbol-1s by zigzag positions; 
% \ao{In reality, because zigzag follows a rough order of frequency (from low to high) and because the blocks are smooth, i.e., low frequency predominates, you will encounter larger values at the beginning of the zigzag, and of course this is why the zigzag is designed this way. This is true even before quantization. Quantization reinforces this effect by using coarser step size for high frequencies.}
% 2) if we look at a small area of an image, e.g., the coding unit of 8x8 block, it must be visually smooth inside the block, which means that after observing some coefficients inside current block, smoothness can help us predict incoming coefficients\xx{I want to say that this prediction is in ``probability sense'', i.e., prediction can't be 100\% sure, not sure what's the correct wording.}; 
% \ao{ Theoretically the coefficient values are not correlated (under some conditions), so I'm not sure what exactly this context is measuring. Following the example you have in Fig. 6, it may be that what is unlikely, and thus penalized by the code, is having a series of very small coefficients followed by a large coefficients. One way to describe this is as follows: item 1) is based on the information that zigzag position provides for any block, independent of the exact contents: average size decreases with position in the zig-zag scan. Instead item 2) says that the pattern of cumulative energy within the block is also predictable, i.e., decrease in energy up to a zig zag scan position in the block predicts decrease in energy from that point forward also, so you expect energy to decrease at predictable rates, very fast in some blocks, not so fast in others. You are not predicting specific coefficient values, rather energy decrease rates, I think. }
% 3) it also has to be similar to nearby blocks, showing that we can use nearby blocks to predict current block.
% \ao{This is easy to explain: Because 8 by 8 is small relative to the size of the images, in each "region" of the image having some characteristics (smooth, texture, etc) there will tend to be several blocks, and so the characteristics of a specific block will be on average related to those of its neighbors.}

% We also need to derive Huffman tables for each context. The goal is to make derived Huffman tables work well for all kinds of images, which means that \sysname needs to get commonly reliable statistical characteristics of symbol-1s for each context. In that way, \sysname does not need to attach tables to each individual image, instead, tables become part of \sysname coder. To achieve this, \sysname trains and derives those Huffman tables from a large image training set. It remains unclear that whether such design works well for images that are outside of the training set, we will answer this question in Section~\ref{sec:eval}.

% In the rest of this section, we first discuss three properties we use to define context, followed by detailed steps for deriving Huffman tables for different contexts.

\subsection{Additional Details}


% We categorize symbol-1s into different contexts. We use three properties to determine context. Before encoding a symbol-1, we calculate beloW three properties of it, and using such three values to determine the context and then use corresponding Huffman table to encode it.



% \subsubsection{Zigzag Position}
% \label{sec:zigzag_position}

% Different zigzag positions represent different frequencies, therefore the distribution of AMPLITUDE on different zigzag positions differ. Besides, JPEG quantization step keeps more information for low frequency energies than high frequency energies: large coefficients occur more at the beginning of zigzag positions (low frequencies) than the end (high frequencies). Figure~\ref{fig:position_distribution} plots the probability of appearance of coefficients that are SIZE 3 on different zigzag positions \footnote{The probabilities are derived from a hundred 600x600 images with quality factor 75. We use the same image set for other plots by default.} We can see that SIZE 3 coefficients occur a lot at zigzag positions 2-10, but occur rarely after zigzag position 20. This indicates that probabilities of symbol-1s of SIZE 3 are different for different zigzag locations. Figure~\ref{fig:position_symbol_distribution} illustrates the probabilities of symbol-1 (RUN 0, SIZE 3).\xx{we may want to put Figure~\ref{fig:position_distribution} and Figure~\ref{fig:position_symbol_distribution} together.} Another example is the End-of-Block symbol. From Figure~\ref{fig:position_0_distribution}, we can clearly see that EOB symbol occurs more at high frequency positions. Both above examples show that the distributions of symbol-1s at different zigzag locations differ and different zigzag position shoud map to different context.

% \subsubsection{Intra-Block Energy Value}
% \label{sec:intra_value}

% \ao{It's not obvious to me what an "unnatural" block is, and I don't think the corresponding images, Fig 6, add much, so I would suggest discussing what smoothness means, and removing Fig. 6}
% The coding unit, 8x8 pixels, is a pretty small area (and in particular for images that have very high resolution, of the order of millions of pixels). Such small areas of the real world images (so called, natural blocks) show some smoothness. Figure~\ref{fig:unnatural_block} (a) shows a block from a real world image and Figure~\ref{fig:unnatural_block} (b) shows a fake block made up by changing its coefficients. By analyzing coefficients of blocks from real world images, we observe that the coefficients of different frequencies are not independent: a natural block spans a similar energy levels to numerous frequencies. On the contrary, if a block only contains high energy for some particular frequencies but no energy for other frequencies, then it will show some strange ``grid''-like pattern (Figure~\ref{fig:unnatural_block} (b)), and we rarely see ``unnatural blocks'' in real world images.

% \ao{changed the beginning here, since we are not computing energy, and instead using a proxy for it. We could even give them different names.}

\parab{Computing intra-block energy.} 
While position information is easily determined, computing the actual
energy would require more computation. To avoid this, we use
alternative quantities to estimate intra- and inter-block energies
that determine context.  We define \emph{intra-block energy} as the
average of the observed coefficient
% %values
% \ao{originally this said values, but in reality we use sizes, which I think is a good idea}
sizes in this block. Let $b_{n}$ denote the $n$-th block, and
$b_n(i)$ denote the coefficient at position $i$. For a given \syma
that occurs at zigzag position $p$, its intra-block energy value is
calculated as:
\begin{equation}
intra(n,p)=\frac{1}{p-1}\sum_{i=1}^{p-1}\frac{SIZE(b_n(i))}{max_{SIZE}(i)}
\label{formula:intra}
\end{equation}
where $SIZE(\cdot)$ denotes the bits required to represent the
amplitude of the coefficient, $max_{SIZE}(i)$ is observed maximum
coefficient size for position $i$ of images in the training set.
%\ao{added below. Xing: see if you agree}
%\xx{agree.}
In theory, the maximum size is the same at any coefficient, but large
sizes may never occur in any of the high frequency coefficients in a
typical dataset. Using $max_{SIZE}(i)$ as a normalization factor
provides a better way to calibrate the significance of an observation:
for example observing a coefficient of size $5$ at position $30$ will
add more to our energy estimate than if the same coefficient was
observed at position $5$, since large sizes are much less likely at
higher positions.

% In other words, $intra(n,p)$ basically averages the size of coefficients 
% before this \syma in this block (weighted by
% $\frac{1}{max_{SIZE}}$ to let high frequency coefficients contribute
% equally as of low frequency coefficients). Intuitively, larger
% $intra(b,p)$ value expects larger SIZE of incoming symbol-1 and vice
% versa.

\parab{Computing inter-block energy.}
For a \syma that happens at position $p$ of the $n$-th block, we
define \textit{inter-block energy value} as the average energy of $F$
similar frequencies in $B$ adjacent prior blocks.  Specifically, this
calculation averages coefficients at positions $p$, $p+1$, $\cdots$,
$p+F-1$ of blocks $b_{n-1}$, $b_{n-2}$, $\cdots$, $b_{n-B}$:
\begin{equation}
inter(n,p)=\frac{1}{B\cdot F}\sum_{i=n-B}^{n-1}\sum_{j=p}^{p+F-1}\frac{SIZE(b_i(j))}{max_{SIZE}(j)}
\label{formula:inter}
\end{equation}
This relies on the smoothness assumption that, if neighboring
frequencies at position $p$ in adjacent blocks have high energy, then
the coefficient at position $p$ in the current block is more likely to
have high energy as well.  We use $F=5$ and $B=3$ in
\sysname.%\rg{What values of $F$ and $B$ do we use?}

% \subsubsection{Context for DC Difference}

% In additional to AC symbol-1s, we also define contexts for encoding DC difference. Nearby blocks have similar DC changes. For example, if previous two DC differences are all 0, it indicates that nearby blocks have similar color and it is reasonable to guess that current DC difference would be a small number as well. We only calculate one property for DC difference context, \textit{inter-block DC changes} (use $b_n(0)$ to denote the DC difference):

% \begin{equation}
% dc(n)=\frac{1}{B}\sum_{i=n-B}^{n-1}\frac{SIZE(b_i(0))}{max_{SIZE}(0)}
% \end{equation}

% \ao{Please see my comments about notation consistency.}


% \subsection{Additional Symbol-1s}

% JPEG groups different coefficients together and does not differentiate those grouped coefficients in symbol-1s. For instance, coefficients 2 and coefficients 3 are grouped together to SIZE 2 coefficients, and coefficients 4, 5, 6, 7 are grouped to SIZE 3 coefficients. Such grouping assumes that coefficients in the same group have similar occurrence probability, and by grouping them together the coding becomes simpler since it has less symbol-1s.

% In our case, because we have finer contexts, for some context we observe that, e.g., probability of coefficient 2 is quite different to the probability of coefficient 3, meaning that grouping them together becomes less efficient. To tackle this inefficiency, we make separate symbol-1s for coefficient 2,3,4,5,6,7. So instead of only having (RUN X, SIZE 2) and (RUN X, SIZE 3), we have (RUN X, COEFFICIENT 2), (RUN X, COEFFICIENT 3), ..., (RUN X, COEFFICIENT 7). For coefficients larger than 7, we still use JPEG's grouping since the probability difference is not as much as small coefficients.

% In addition to AC symbol-1s, we also double the symbol-1s of encoding DC difference, by adding the sign of DC difference as part of the symbol-1s. For example, instead of having (SIZE 1), we have (SIZE 1 Positive) and (SIZE 1 Negative). The reason of doing this is that we observe for some contexts, the probability of having positive DC difference versus having negative DC difference is not fifty-fifty.

\parab{Learning the context-sensitive Huffman tables.}
\sysname generates a Huffman table for each specific context from a
training set of images. For each \syma that occurs in any image in the
training set, \sysname can determine its context: $p$, $intra(n,p)$
and $inter(n,p)$. Since the latter two quantities are real-valued,
\sysname quantizes these values into $U$ buckets. Buckets are sized so
that each bucket contains the same number of \symas. Thus, $U$ is a
parameter in \sysname that trades-off the size of the Huffman tables
for increased discrimination by context. In our experiments, we use
$U=20$.

Thus, after quantization, a context in \sysname is a triple
$<p, i, e>$, where $i$ denotes the intra-block bucket index, and $e$
the inter-block bucket index.  From the training set, for each unique
$<p, i, e>$, \sysname can generate a table of \symas seen with that
context, and the number of occurrences of each \syma.
% \ao{I would
%   suggest adding to the caption of Table~\ref{tbl:table_comparison} so
%   that it is easier to get some intuition from it. This could be done
%   in the caption or in the text here. What I would like to see is why
%   the results of Context A and Context B are reasonable, given what
%   those contexts are. }
% \xx{done}
Table~\ref{tbl:table_comparison} shows such a table for two different
contexts, derived from a training set of 100 images: notice how
different these tables are. From these tables, \sysname generates
Huffman encodings for different \symas using a standard
procedure~\cite{huffman}.
Some \symas may never be observed during training, but can occur when
encoding an uploaded image. \sysname assumes that all unseen symbols
are equally likely and occupy a small, fixed, probability mass. This
works well in practice (Section~\ref{sec:eval}).

% We derive those tables based on images of the training set. We extract all the symbol-1s from the training set and make three passes of it. The first pass records the $max_{SIZE}$ information of the training set. The second pass separates the value range of both intra-block energy value $intra(n, p)$ and inter-block energy value $inter(n, p)$ into $U$ buckets and thus maps both real number values into integers (bucket number). There are infinite ways of separating their value range $[0, 1]$, we separate it by making each bucket contain roughly the same number of symbol-1s.

% The third pass actually derives the Huffman tables. We call a
% combination of three properties (in total $63\times U\times U$
% combinations) a context. Given the output of the first and second
% passes, for each symbol-1, we know exactly which context it belongs
% to. For each context, we gather all the symbol-1s that belong to
% this context together, and derive the optimal Huffman table based on
% the occurrence probabilities of different symbol-1s. Such optimal
% Huffman table can represent symbol-1s of this context in least
% bits. Explained earlier in this section, we list the most frequent
% occurred symbol-1s of two contexts in
% Table~\ref{tbl:table_comparison}\footnote{For this example we make
% 20 buckets for both $intra(\cdot)$ value and $inter(\cdot)$ value
% ($U$ = 20).}.

% \ao{The statement below is very unclear. What is standard is to use this idea to update the probabilities of things that have not been seen, but are you saying your tables cover all the possible cases, but with very low probability, long codewords, for things that have not been seen in the training set? You are no longer doing escape codes and the like?}
% This is a standard problem in designing
% adaptive encoders, and an accepted way of dealing with this (which
% \sysname also uses) is to assume that each unseen symbol occurs at
% least once in the training set.

% We need to make sure that trained Huffman tables can encode any image. It means that, 1) each context's Huffman table can encode any possible symbol-1, even if such symbol-1 never occurs in such context in the training set; and 2) we need to have a Huffman table for each context, even if we have not observed any symbol-1 in that context in the training set. For 1), we give the combination of all the symbols that have not occurred a probability of $P\%$\footnote{Intuitively, $P\%$ depicts the incompleteness of the training. It is determined by calculating the probability of training set's missing symbol-1s in a large enough testing set. A typical $P\%$ we see is roughly $1\%$}. For example, assume there are 10 symbol-1s that have not appeared in the training set, we assume that each one of these 10 symbol-1s occurs with probability $P\% / 10 = 0.1P\%$. For 2), we train a default Huffman table, which reflects the symbol-1s' overall probability across the entire training set and use that for the contexts of 0-observation.

\parab{Encoding and Decoding in \sysname.}
After the Huffman tables are trained, \sysname can encode uploaded
JPEG images losslessly (Figure~\ref{fig:sysname}). For an uploaded
image $I$, \sysname's encoder applies the standard JPEG \emph{decoder}
on $I$ to obtain the quantized DC coefficients in each block of $I$.
For each \syma in each block of $I$, \sysname computes its $<p,i,e>$
context, then represents \syma using the corresponding code from that
context's Huffman table.

% With the trained Huffman tables ready, Figure~\ref{fig:sysname} illustrates how \sysname encodes a given JPEG image losslessly. \sysname uses standard JPEG entropy decoder to get blocks of DCT coefficients. Then it encodes those DCT coefficients using our context sensitive entropy encoder, by first generating symbol-1s (\sysname uses extra symbol-1s so this generation step is similar but not completely identical to JPEG), and then for each of them, calculating its $p$, $intra(\cdot)$ and $inter(\cdot)$ to determine which context it belongs to and using Huffman table for that context to encode this symbol-1.

When decoding an image before transmitting to a client, \sysname can
calculate the $<p,i,e>$ context for the \syma (since this depends on
already decoded symbols), then does an inverse lookup on that
context's Huffman table to find the $(k,l)$ representation of the
\syma. After all symbols have been decoded, \sysname uses the standard
JPEG entropy \emph{encoder} to generate the original JPEG image. In
large photo sharing services, this original JPEG may be subjected to
other transformations before being downloaded to clients. 

% Similarly, in \sysname's decoder, when it is about to decode a symbol-1, it calculates the current $p$, $intra(\cdot)$ and $inter(\cdot)$ to find the correct Huffman table to decode the incoming symbol-1. After decodes all the coefficients, \sysname just uses standard JPEG encoder to recover the original JPEG image.

% This design has several interesting properties. Because it can recover
% JPEG images completely, it can be transparently interposed into any
% existing pipeline after all JPEG transformations on the upload path
% (e.g., a photo sharing service might reduce image quality of an
% uploaded image), and before all JPEG transformations on the download
% path (e.g., resizing an image or transcoding to a different format
% before downloading). Moreover, \sysname works on DCT coefficients
% directly, never de-quantizes them nor transforms them back to the
% pixel domain, which is one of the reasons why \sysname achieves
% minimal increase in computational complexity.

% In this section, based on the idea of separating contexts and deriving
% Huffman tables for different contexts, we propose \sysname to
% represent JPEG images more efficiently in bits. \sysname uses trained
% Huffman tables to encode and decode JPEG images. \sysname is a
% lossless representation of JPEG images.

% RG: For this audience, probably OK to omit. If reviewed by a signal
% processing person, they will likely appreciate that we handled these details.
% \ao{Is it ok to explicitly omit these details? It may be better to at
%   least say something about how this is done, for example how
%   something we omit is similar to something we described. }

\parab{Omitted details.} For brevity, we have omitted some details of
the entropy coder in \sysname, including: determining the context for
DC coefficients using the difference in DC coefficients between
neighboring blocks; encoding the sign of this DC coefficient
difference in the \syma; generating additional \symas beyond the ones
used in JPEG in order to make finer-grain distinctions in the
probability of occurrence, especially at lower frequencies. These
extensions generalize the definition of \symas in ways beyond encoding
run-lengths and coefficient sizes, but help generate Huffman tables
that improve compressibility.

% The design section title often includes the name of the system.  The
% section itself is often the longest and hardest to write.  One
% particularly tricky aspect is figuring out what to include and in what
% order.  Often we will describe the most basic version of the system
% first and then describe extensions/optimizations/complications in a
% separate section or subsection.

% \begin{figure*}[t]
% \centering
% %\includegraphics[width=1.0\linewidth]{figs/arch-crop}
% \placeholderwide{You can put what you think should be in the figure
%   here before you make it.\\

%   A common way to make these figures is to use powerpoint to draw the
%   figure, save it as a pdf locally, and then crop it using 'pdfcrop
%   -{}-margins 1'.  You should save the pptx and pdf files in the /figs
%   subdirectory.}
% \caption{The architecture of System.}
% \label{fig:arch}
% \end{figure*}

% %% For pseudocode and other figures it is often better to put them in
% %% their own file and then input them so you don't break up the flow
% %% of the .tex file too much.
% \input{eiger_read_only_txn_algo.tex}
% %\input{algpseudocode.tex}

% The design section often includes an architectural diagram like the
% one in Figure~\ref{fig:arch}.  It also often includes psuedocode like
% what is in Figure~\ref{pc:read_txn}.


% \subsection{Extensions}
% \label{sebsec:ext}

% Subsections are a great way to organize longer sections.  If you want
% another level of organziation use {\textbackslash}paragraph\{\}
% instead of {\textbackslash}subsubsection\{\}.


==> codec_lossy.tex <==
\section{A Gracefully Lossy Coder}
\label{sec:codec_lossy}

% \ao{ A Graceful Codec sounds odd. Maybe: A Lossy Coder Providing Graceful Degradation? Basically what's graceful is the quality degradation, not the codec. Or Gracefully Lossy? }

\sysname's entropy coder is lossless with respect to the uploaded
JPEG. In this section, we describe \lossyname, which introduces loss
(or \emph{distortion}) in uploaded images as a way of achieving
further savings in photo storage. % \lossyname more gracefully degrades
% perceptual quality than other alternatives for introducing loss.

\parab{Motivation.} As discussed in Section~\ref{sec:integrating},
some photo service providers change the JPEG quality parameter in
uploaded images in order to ensure predictable storage usage, a step
that introduces distortion~\cite{coulombe2010transcoding}.
%
% Camera device resolutions have increased dramatically in recent years,
% and uploaded image sizes have been increasing steadily. To control
% storage usage, providers have at least two tools available to them:
% re-scaling the image to a smaller size, and changing the
% \emph{quality} of the image. Both of these can introduce distortion,
% but are necessary tools to combat the scaling problems photo sharing
% services face. See \cite{coulombe2010transcoding} for a discussion of
% transcoding an uploaded by changing both size and quality.
%
% As
% discussed earlier, many JPEG tools provide ways to control image
% quality using QP (a single value between 0 and
% 100 chosen for the whole image). 
% \ao{This repeats what was said in the JPEG section and could be shortened}
% Effectively, this quality parameter controls the quantization
% step size~\cite{jpeg_still}: lower values increase the denominator
% (the quantizer), so more of the least significant bits are dropped.
%
To achieve this, a photo storage service has to decode the
coefficients from the uploaded image, and \emph{re-quantize} the
coefficients. In contrast, the camera that generated the image in the
first place applies the quantization to the original coefficients.

Figure~\ref{fig:better_transcoding} shows that re-quantizing can cause
images to be distorted less gracefully than applying the same degree
of quantization on the original image\footnote{We use the
  \texttt{convert} tool of ImageMagick \cite{imagemagick} for image
  transcoding.}. The figure plots a metric of image perceptual
quality, the peak signal-to-noise ratio (PSNR) \cite{psnr} against
image size, obtained by changing the quality factor on all images in a
collection of 100 images. The ``Changing Quality from Raw Image'' curve is obtained by
reducing the quality factor when compressing the original raw images,
while the ``Changing Quality from Uploaded JPEG'' curve is obtained by
re-quantizing a high-quality JPEG image derived from the same set of
raw images. The former curve represents much more graceful
degradation.
%a nearly linear relationship between distortion and size
%reduction. 
By contrast, re-quantization introduces much more
distortion for the same size reduction. This is because
the JPEG quantization step uses floating point arithmetic
% \xx{There is only integer calculation if it's re-quantizing follow $\parallel \parallel c \times q_{old} \parallel \div q_{new} \parallel$.}
% \ao{I don't understand your comment: wouldn't you need floating point or some fixed point arithmetic for the division? }
and involves an integer rounding step at the end, since the quantized
coefficients are represented using integers. Re-quantization adds an
additional rounding, resulting in increased distortion relative to
applying quality factors to the raw images.

\parab{Our Approach.}
\lossyname avoids re-quantizing coefficients, but introduces
distortion by carefully setting \emph{some} non-zero (quantized)
coefficients to zero, a specific instance of a general idea called
thresholding~\cite{thresholding}. While more generalized forms of
thresholding have been explored in other contexts, we are not aware of
it being explored as an alternative to re-quantization in large photo
sharing services.  The intuition behind thresholding is that, by
setting a well-chosen non-zero coefficient to zero, it is possible to
increase the number of consecutive zero-valued coefficients in the
sequence of linearized coefficients. This helps reduce size because
the entropy coder compresses a run of zero-valued coefficients into a
run-length.

How to choose which coefficients to threshold? Intuitively, the right
choice is one that minimizes the distortion while maximizing the
storage reduction. This can be quantified using a ratio of bits-saved
to distortion or by introducing a Lagrangian cost function
\cite{ortega1998rate,thresholding}.  Recall that in the JPEG entropy
encoder, each non-zero coefficient is represented by a \syma.
By setting a non-zero coefficient to
zero we save bits required to represent that \syma. However, this step
introduces distortion. In this paper, we demonstrate the efficacy of a
simple strategy: whenever the ratio of the bits-saved to
induced-distortion for a non-zero coefficient is greater than a
threshold $\tau$, set that coefficient to $0$.

Computing the bits-saved is straightforward: for a given coefficient,
thresholding replaces two \symas with one, and we can compute the
number of bits required for the original \symas and the new \syma by
looking up the appropriate context-sensitive Huffman tables of
\sysname. The difference between the two quantities represents the
bits-saved by thresholding that coefficient.

One way to compute the induced-distortion would be to transform the
image back to the pixel domain, and compute the resulting quality
metric (say, PSNR). The drop in this metric would then be a measure of
distortion. However, each pixel domain conversion can be
computationally expensive.

\lossyname uses two mathematical properties to simplify this
calculation. First, the DCT transform is orthogonal, so any distortion
in the frequency domain is identical to a distortion in the pixel
domain. Thus, we do not need to transform the image back to the pixel
domain. Second, many image quality metrics compute the mean-squared
error (MSE) with respect to the original image. Removing a coefficient
$A$ increases the MSE by:
$((quantizer\ of\ A)\times(amplitude\ of\ A))^2$ so the induced
distortion can be calculated easily using this formula. Such
calculations can be extended to other metrics like SSIM (Structural
Similarity Metric~\cite{ssim}) which we have left to future work.

% \lossyname estimates the
% additional distortion of removing one DCT coefficient. Additional
% distortion can be calculated easily in pixel domain, \lossyname needs
% to estimate distortion fast and thus we design it to stay in DCT
% domain for distortion estimation. There are different choices of
% distortion metric, we use Peak-Signal-to-Noise-Ratio (PSNR)
% \cite{psnr} for \lossyname. PSNR is based on Mean Squared Error (MSE)
% \cite{mse} calculation, so \lossyname needs to estimate the MSE change
% after removal of one DCT coefficient, A, via formula:



% \ao{In terms of terminology: what changes is the quantization stepsize, not the quantizer. You could say that the quantizer changes also, but it's typical to say you change the quantization parameter. So, change to quantization parameter.  }\xx{in ``jpeg still'' paper, it uses quantizer as the quantization factor of each frequency, so one quantization table contains 64 quantizers. I'll fix terminology later.}

% In Formula~\ref{formula:distortion}, \lossyname gets the de-quantized DCT coefficient of A by multiplying it by the quantizer of A's frequency, which is the coefficient value we set to zero (error), and then it computes the square to get MSE change in DCT domain. Since the DCT is an orthogonal transform the MSE change in DCT domain is equal to the MSE change in pixel domain, in this case, we calculate the MSE change of removal of A accurately.

% \ao{The transform is orthogonal, so distortion is the same in the transform and pixel domain}


% Similar DCT domain distortion estimation can be applied on other distortion metrics. For example, \cite{ssim_distortion} explains how to calculate Structural Similarity (SSIM) distortion metric \cite{ssim} in DCT domain.


% we can drop two symbols representing this DCT
% coefficient and thus save some
% bits. %\ao{Both removal and modification introduce distortion}
% The removal of non-zero DCT coefficients introduces distortions. The
% choice of removing a non-zero DCT coefficient or not should take into
% account both bits-saving and distortion information. For any DCT
% coefficient, \lossyname accurately estimates 1) the bits-saving and 2)
% the distortion of removing it, and generally removes the DCT
% coefficients of good bits-saving and small distortion. \lossyname
% computes the \emph{ratio of bits-saving and distortion} and uses a
% \emph{threshold} to quantify whether one DCT coefficient should be
% removed or not.

% In this section, we propose \lossyname, a lossy variant of \sysname, for image-sharing service providers who want to further compress images without the strict lossless constraint. \lossyname uses the same entropy coder of \sysname, with an \emph{block-modification} step added before entropy encoding step (Figure~\ref{fig:sysname}), which modifies blocks in DCT domain for additional bits-saving. \lossyname leverages idea from \cite{thresholding}, which picks and sets non-zero DCT coefficients to zero and minimizes the distortion of doing so for a given bits-saving budget. \lossyname uses a simpler and thus faster approach, it enumerates non-zero DCT coefficients sequentially, estimates the distortion as well as the bits-saving  introduced by setting each coefficient to zero, and decides whether set such DCT coefficient to zero or not independently from decisions of other non-zero coefficients. This approach achieves the same optimization goal of \cite{thresholding} approximately.

% \begin{figure}
% \centering
% \begin{minipage}[t]{0.45\textwidth}
% \includegraphics[width=\columnwidth]{exps/lromp_vs_quant/lromp_vs_quality2.pdf}
%   \caption{\lossyname vs. Requantizing}
%  \label{fig:lossy_transcoding}
% \end{minipage}
% \end{figure}

% \lossyname can modify JPEG images in a perceptually-lossless manner, by only modifying DCT coefficients that would not introduce perceptual distortion\xx{actually we don't know what is a perceptual distortion for each thresholding, we know the error it introduces though. so we should say ``introduce small distortion'' to be honest}. Conceptually, this is similar to lower the quality parameter a bit for the uploaded image whose quality parameter is high, however, traditional quality parameter changing approach, which decodes the image and re-encode it using a lower quality parameter, introduces significant error, shown in Figure~\ref{fig:lossy_transcoding}. The black curve (Raw Image) shows the rate-distortion curve of transcoding from the raw image to different quality parameter. Other color curves show the results of lowering quality parameter from a JPEG image (the uploaded image) of different quality parameter. We see a big PSNR drop\footnote{Such error is generated by the two integer rounding calculations in JPEG quality parameter changing process, which needs to de-quantize the DCT coefficient, $c$, using the old quantizer, $q_{old}$, and then quantize it again using the new quantizer, $q_{new}$: $\parallel \parallel c \times q_{old} \parallel \div q_{new} \parallel$.} comparing to the curve of transcoding from raw image, especially when the desired quality parameter is close to the quality parameter of the uploaded JPEG, meaning that traditional approach deviates from original image significantly. In Section~\ref{sec:eval}, we will show that \lossyname does a much better job, tracks the curve of trancoding from raw image nicely. Below we introduce how to select coefficients to set to zero in detail.

% \ao{I modified the above. There are a couple of issues with the 2nd bullet. 1) Our approach is better than changing the QP parameter by decoding a quantized image and re-encoding it. There is significant loss associated to that process, but as we saw in the experiments encoding the original image at a different QP is Ok. 2) There are some limitations in thresholding: it is only efficient for small changes in RD. As you decrease the threshold, or threshold larger values, i.e., not only 1 but 2, 3, etc, you can deviate significantly from the original JPEG RD curve.}

% \subsection{Compute Ratio of Bits-Saving and Distortion}

% \ao{We need to provide some context for the idea of thresholding, in particular the paper by Ramchandran and Vetterli }\xx{added a sentence in above paragraphs. also state the difference, please take a look. and I implied our approach considers setting to 0 only, so below I won't talk about ``modification'', only ``zero-off'' then.}

% In the JPEG entropy encoder, each non-zero DCT coefficient needs a pair of symbols (Table~\ref{tbl:inter_symbols}) to represent. By setting one non-zero DCT coefficient to zero (in other words, removing it), we can drop two symbols representing this DCT coefficient and thus save some bits. %\ao{Both removal and modification introduce distortion}
% The removal of non-zero DCT coefficients introduces distortions. The choice of removing a non-zero DCT coefficient or not should take into account both bits-saving and distortion information. For any DCT coefficient, \lossyname accurately estimates 1) the bits-saving and 2) the distortion of removing it, and generally removes the DCT coefficients of good bits-saving and small distortion. \lossyname computes the \emph{ratio of bits-saving and distortion} and uses a \emph{threshold} to quantify whether one DCT coefficient should be removed or not.

% \begin{table}
% \centering
% \begin{tabular}{ l l l}
%   \textbf{Before} & $\cdots$; \emph{(RUN 3, SIZE 1), 1}; (RUN 0, SIZE 2), 2&;$\cdots$\\
%  \textbf{After}  & $\cdots$; (RUN 4, SIZE 2), 2&;$\cdots$\\
% \end{tabular}
%   \caption{Removing of DCT Coefficient}
%   \label{tbl:removal}
% \end{table}

Finally, \lossyname can be easily introduced into \sysname's
pipeline. After quantizing each block, but before applying the
context-sensitive entropy coding, \lossyname's thresholding can be
applied to each block (Figure~\ref{fig:sysname}). No changes are
required to \sysname's entropy coder.

% The question of whether, when, and to what extent a photo sharing
% service should distort images is a \emph{policy} question that can
% only be formulated based on experience from actual deployments, so we
% have left this to future work. Generally speaking, photo services will
% want to induce distortion that leaves perceptual quality
% unchanged. 
% \ao{I feel the statements here are too weak. I think it is possible to introduce thresholding that does not introduce any perceived distortion. I think we should make a stronger case that at the very least zero perceptual distortion thresholding should be possible. }
% This is possible to do: modern cameras generate images of
% high enough quality that services can induce small distortions without
% affecting perceptual quality. However, understanding what values of
% $\tau$ to use for a given quality of an upload image is beyond our
% scope and left to future work.

% \subsubsection{Estimate Bits-Saving}

% \ao{I think the discussion below could be simplified: the JPEG entropy coder encodes a series of zeros followed by a non-zero. if we replace a non-zero by a zero, this either creates an EOB or it makes the zero run before the next non-zero coefficient longer. This is all clear from the structure of the JPEG entropy coder. }

% To estimate the bits-saving of removing one DCT coefficient of a block, the naive approach would be to calculate the bits difference of representing current block and the block after removal of such coefficient. Instead, we note that it is only necessary to consider the symbols representing this DCT coefficient (we call it A for simpler explanation) and the next non-zero DCT coefficient (we call it B) to compute the bits-saving. Because symbols of DCT coefficients before A and symbols of DCT coefficients after B would not be affected. Generally, the removal of A involves removing of symbols representing A and updating the symbol-1 of B. We illustrate an example in Table~\ref{tbl:removal}, where we estimate the bits-saving of removing the emphasized DCT coefficient A, represented by the symbols including symbol-1: \emph{(RUN 3, SIZE 1)} and symbol-2: \emph{1}. There are 3 zeros before A (RUN 3), and no zero before B (RUN 0); after the removal of A, there are 3 zeros plus, A itself becomes zero, and thus in total 4 zeros before B, so we need to update B's RUN to 4. We use below formula to calculate bits-saving of removing DCT coefficient A:
% \begin{align}
% \emph{bits-saving}= &bits(\textbf{symbol-1}\ of\ A) + bits(\textbf{symbol-2}\ of\ A)\nonumber\\
%         &-bits(updated\ \textbf{symbol-1}\ of\ B)
% \label{formula:bitssaving}        
% \end{align}

% Different entropy encoders use different bits for symbols, and thus give different bits-saving results for Formula~\ref{formula:bitssaving}. Ideally, we can use \sysname's entropy encoder to calculate accurate bits-saving. In \lossyname's implementation, to be more efficient in complexity, we use JPEG standard's entropy encoder to estimate bits-saving, since it only uses a single, fixed Huffman table instead of calculating contexts and using different Huffman tables, which reduces the complexity, and also approximates bits-saving result nicely.

% \subsubsection{Estimate Distortion}

% \lossyname estimates the additional distortion of removing one DCT coefficient. Additional distortion can be calculated easily in pixel domain, \lossyname needs to estimate distortion fast and thus we design it to stay in DCT domain for distortion estimation. There are different choices of distortion metric, we use Peak-Signal-to-Noise-Ratio (PSNR) \cite{psnr} for \lossyname. PSNR is based on Mean Squared Error (MSE) \cite{mse} calculation, so \lossyname needs to estimate the MSE change after removal of one DCT coefficient, A, via formula:

% \begin{equation}
% \emph{distortion}=((quantizer\ of\ A)\times(amplitude\ of\ A))^2
% \label{formula:distortion}
% \end{equation}

% \ao{In terms of terminology: what changes is the quantization stepsize, not the quantizer. You could say that the quantizer changes also, but it's typical to say you change the quantization parameter. So, change to quantization parameter.  }\xx{in ``jpeg still'' paper, it uses quantizer as the quantization factor of each frequency, so one quantization table contains 64 quantizers. I'll fix terminology later.}

% In Formula~\ref{formula:distortion}, \lossyname gets the de-quantized DCT coefficient of A by multiplying it by the quantizer of A's frequency, which is the coefficient value we set to zero (error), and then it computes the square to get MSE change in DCT domain. Since the DCT is an orthogonal transform the MSE change in DCT domain is equal to the MSE change in pixel domain, in this case, we calculate the MSE change of removal of A accurately.

% \ao{The transform is orthogonal, so distortion is the same in the transform and pixel domain}


% Similar DCT domain distortion estimation can be applied on other distortion metrics. For example, \cite{ssim_distortion} explains how to calculate Structural Similarity (SSIM) distortion metric \cite{ssim} in DCT domain.

% \subsection{\lossyname Work Flow}

% We describe how to estimate the bits-saving as well as the additional distortion above. Compared to \sysname, \lossyname's additional component, block-modification step, modifies each block sequentially before input to entropy encoder step (Figure~\ref{fig:sysname}) by calculating the ratio of bits-saving and distortion for each non-zero DCT coefficient and removing those whose ratios are higher than threshold. \lossyname uses such threshold to control the tradeoff between bits-saving and distortion to achieve perceptual-lossless for different images.

% \xx{below are my old draft, which is what Antonio commented on. also removed ``two use cases'' in the first paragraph.}
% \ao{I don't think we should separate these two cases. For the type of services we have in mind, it wouldn't make sense to be so aggressive with compression that we create a significant degradation in image quality. I think we would like to be perceptually lossless, or close to lossless, in any case, and being more or less aggressive is a matter of how much we would like to compress. Perceptually lossless basically means that someone cannot see the difference between the original image and the processed one. 
% The main problem is how to define a threshold for perceptually lossless. I think we can think about it in the following way: most images are uploaded at a relatively high quality level, which means that even if they had been coded at slightly lower quality they would have looked similar. Our approach is locally almost the same in PSNR as changing the original QP by one or two levels. So, based on this we could say that if the original QP is good enough (e.g., over 70), then a PSNR loss that is comparable to changing the original QP (from the original image, black curve in Fig 14) by only 1-2 steps is going to be perceptually lossless. }
% \parab{Perceptual-Lossless Compression.} \lossyname can further compress JPEG image in a perceptual-lossless manner, by using a relatively high threshold to only remove DCT coefficients that would not perceptually altering the image. \xx{describe what is percetual-lossless and how do we determine threshold.}

% \parab{Aggressive Lossy Compression.} Some photo-sharing services want to compress uploaded images aggressively. Traditionally this is done by lowering the quality parameter of uploaded images. \lossyname can serve for the same purpose, by using a relatively low threshold, however \lossyname's achieved rate-distortion result can be much better than the traditional approach. Figure~\ref{fig:lossy_transcoding} shows the distortion introduced by the traditional approach that changes the quality parameter. The black curve (Raw Image) shows the rate-distortion curve of transcoding from the raw image to different quality parameter. Other color curves show the result of lowering quality parameter from a JPEG image of different quality parameter. We see a big PSNR drop comparing to the curve of transcoding from raw image, especially when the desired quality parameter is close to the quality parameter of the original JPEG, showing that, without the raw image, changing the quality parameter from uploaded JPEG image introduces significant error. Such error is generated by the integer rounding in JPEG quality parameter changing process, which needs to de-quantize the DCT coefficient, $c$, using the old quantizer, $q_{old}$, and then quantize it again using the new quantizer, $q_{new}$: $\parallel \parallel c \times q_{old} \parallel \div q_{new} \parallel$. In Section~\ref{sec:eval}, we will show that \lossyname tracks the curve of trancoding from raw image nicely, and thus serves aggressive compression purpose better than the traditional approach.

==> design_deleted.tex <==
The most well-known efficient JPEG recompression scheme, PackJPG~\cite{packjpg}, can provide about 20\% additional compression
in photo sizes, but has significant decompression
complexity. Figure~\ref{fig:recompression_at_backend} shows the CDF of
latencies of downloading a 2048$\times$1536 image from the backend, with and without
recompression using PackJPG.\footnote{The methodology for this experiment is
  explained in Section~\ref{collateral}.} % We add 531ms decompression
We see that the recompression %(531ms in this case)
inflates the
latency of the fastest 40\% of downloads by more
than 50\%. Even though the decompression latency is incurred only for
cache misses, we still see significant impact on the overall latency
distribution (from all the layers of the cache stack):
\tld80\% of the distribution incurs more than 150ms additional
latency.  For commercial photo sharing services, these increases in latency may not be acceptable.

% \begin{figure}[t]
% \centering
% \noindent\includegraphics[width=0.7\linewidth]{../pics/plot_edge_fb.eps}
% \shortentablecaptiona
% \caption{Access latency distribution of deploying the decoder at the edge. The 1st subplot shows the access latency before and after the deployment; the 2nd subplot shows the additional latency introduced by decoding for each percentile.}
% \shortentablecaptionb
% \label{fig:recompression_at_edge}
% \end{figure}

These photo services can also reap other benefits of recompression.
For example, in Figure~\ref{fig:download_path}, moving the
decompression and transcoding close to the clients can have two
important benefits.  First, caches would now be more storage
efficient, because they would store recompressed versions of the
photos. This would result in fewer accesses to the backend storage
and caches. Second, the bandwidth required between the caches and the
backend storage would be reduced because only recompressed images
would need to be transferred. However, to reap these benefits, the
additional decompression latency would affect \emph{all the
  accesses}. In this case, low complexity decompression is even more
important: as Figure~\ref{fig:recompression_at_edge} shows, using the
state-of-the-art PackJPG, with its high decompression complexity, can
increase latency by more than \emph{half a second}.


==> eiger_read_only_txn_algo.tex <==
\newcommand\KW[1]{\textbf{#1}} %keyword
\newcommand\CM[1]{\emph{#1}}   %comment
\newcommand\LA{$\gets$}  
\newcommand\INF{$\infty$}
\newcommand\GE{$\ge$}
\begin{figure}[t]
\hrule\ 
\small%
\begin{Verbatim}[commandchars=\\\{\}, numbers=left]
\KW{function} read_only_trans(requests):
  # \CM{Send first round requests in parallel}
  \KW{for} r \KW{in} requests
    val[r] = multiget\_slice(r)

  # \CM{Calculate the maximum EVT}
  maxEVT = 0
  \KW{for} r \KW{in} requests
    maxEVT = max(maxEVT, val[r].EVT)

  # \CM{Calculate effective time}
  EffT = \INF
  \KW{for} r \KW{in} requests
    \KW{if} val[r].LVT \GE maxEVT
      EffT = min(EffT, val[r].LVT)

  # \CM{Send second round requests in parallel}
  \KW{for} r \KW{in} requests
    \KW{if} val[r].LVT < EffT
       val[r] = multiget\_slice\_by\_time(r, EffT)

  # \CM{Return only the requested data}
  \KW{return} extract_keys_to_columns(res)
\end{Verbatim}
\hrule\ 
\caption{Pseudocode for Eiger's read-only transactions.}
\label{pc:read_txn}
\end{figure}


==> old_fiture_placement.tex <==
\begin{figure*}
\hspace*{\fill}
\centering
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/tecnick_vs_quality/tecnick_vs_quality_final.pdf}
\caption{The compression ratio as the quality parameter increases (1200$\times$1200).}
\label{fig:tecnick_quality}
\end{subfigure}
\hfill
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/tecnick_vs_resolution/tecnick_vs_resolution_final.pdf}
\caption{The compression ratio as the resolution increases (quality parameter is 75).}
\label{fig:tecnick_filesize}
\end{subfigure}
\hspace*{\fill}
\caption{The compression ratio over JPEG Standard as quality parameter and resolution changes for Tecnick image set. Competitors are: \sysname, \lossyname, \aggrename, JPEG Optimized (OPT), JPEG Progressive (PRO), JPEG Arithmetic (ARI), MOZJPEG (MOZ) and PackJPG (PJG).}
\end{figure*}

\begin{figure*}[t]
\hspace*{\fill}
\centering
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
    \caption{1152$\times$864, quality parameter is 75}
    \label{fig:fivek_tradeoff-1}
\end{subfigure}
\hfill
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/comp_vs_quality/comp_vs_enc_2048_final.pdf}
    \caption{2048$\times$1536, quality parameter is 75}
    \label{fig:fivek_tradeoff}
\end{subfigure}
\hspace*{\fill}
\caption{Compression/complexity trade-off of FiveK image set, with quality parameter of 75 at 2 different resolutions. Encoding complexity is marked in red and decoding complexity is marked in blue. Competitors are: \sysname, \lossyname, \aggrename, JPEG Optimized (OPT), JPEG Progressive (PRO), JPEG Arithmetic (ARI), MOZJPEG (MOZ) and PackJPG (PJG).}
\end{figure*}


\begin{figure*}[t]
\hspace*{\fill}
\centering
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/coding_vs_time/dec_vs_time.pdf}
    \caption{The decoding complexity as quality parameter increases (1200$\times$1200).}
    \label{fig:complexity_quality}
\end{subfigure}
\hfill
\begin{subfigure}{\subfigurewidth}
  \centering
\includegraphics[width=\twocolumnfigurewidth]{../exps/time_vs_res/fib_9b.pdf}
    \caption{The decoding complexity as resolution increases (quality parameter is 75).}
\label{fig:complexity_coding}
\end{subfigure}
\hspace*{\fill}
\caption{The decoding complexity as quality parameter and resolution changes for Tecnick image set.}
\end{figure*}

==> recompression_backup.tex <==
\section{Low-Complexity Recompression for Photo Sharing Services}
\label{sec:romp-lromp}
\label{sec:recompression}

In this section, we
discuss the design of ROMP and L-ROMP, which recompress JPEG images to reduce the storage requirements of large-scale photo sharing services significantly with low complexity overhead. Before doing this, we briefly
describe the JPEG standard; our description is highly simplified and
omits many details~\cite{jpeg_still}.

\subsection{The JPEG Standard}
\label{sec:background}

Each digital image compressed using the JPEG standard is divided into
contiguous, non-overlapping blocks of $8\times8$ pixels. As a first
step, each block of pixels is transformed using the Discrete Cosine
Transform (DCT)~\cite{dct}, generating as an output $64$
frequency-domain {\em transform coefficients}, each representing
information at a different frequency within the block.
JPEG compression performs quantization and entropy coding for each of
these image blocks.  

First, transform coefficients are \emph{quantized} by truncating a
selected number of least significant bits. This is a lossy step
and will lead to distortion in the reconstructed image with respect to
the original one. The amount of quantization is controlled by a
\emph{quantization table}, which determines the relative amount of
quantization to be applied to each frequency within a block, and by a
\emph{quality parameter}, which is used to control the overall image
quality by adjusting quantization across all coefficients of all
blocks.  These two parameters combined together determine the
actual quantization applied to a given transform coefficient.  In
general the quantization table assigns different levels of
quantization to each of the 64 coefficients, so as to introduce more
losses in the high frequencies than in the low frequencies. This has
been shown to be more efficient as quantization errors in the higher
frequencies are less visible to the human eye (in this sense, such
transformations are said to be \emph{perceptually lossless}). In a
typical software implementation, the quality parameter is a number
between 1 and 100, with lower values indicating coarser quantization
(more least significant bits truncated) resulting in more compression (smaller file
size) at the cost of increased loss (worse quality of the
reconstructed image). This parameter affects all image blocks in the
same way.

After quantization, the information in each block consists of a series
of integer values representing the quantized coefficients. These
integer values are mapped to uniquely decodable variable length codes
for storage. In this {\em entropy coding} process the basic principle
is to assign shorter codes to coefficient values that are more likely,
resulting in overall lower bit rate. For typical images the DCT
coefficients after quantization tend to be ``sparse'' (i.e., many of
them are likely to be zero) and often localized in the low frequencies
(i.e., the higher frequency coefficients are more likely to be
zero). JPEG exploits this by encoding transform coefficients in a block
following a sequential ``zig-zag'' scan, in rough order of decreasing
frequency. Thanks to this, coefficients along the zig-zag scan tend to
have decreasing size. When all remaining coefficients in a block are
zero, an end-of-block code is sent. This scan order favors the
early occurrence of an end-of-block, resulting in greater compression
efficiency.

Because zeros are likely to occur, they are grouped before entropy
coding by using \emph{run-length encoding}: replacing each contiguous
sequence of zeros along the zig-zag scan with a run-length, an integer
indicating the number of consecutive zeros.  In the last step,
\emph{entropy-coding}, the length of a run and the value of the
following non-zero coefficient are mapped to a uniquely decodable
codeword. This mapping of input integers representing run-length and
quantized coefficient values (or \emph{symbols}) into variable length
bit string is represented by a \emph{Huffman table}.

While it is possible to customize quantization and Huffman tables,
many JPEG implementations make use of widely agreed on ``default''
tables.  Thus, in practice, these tables need not be included with
each image (e.g., when an image is uploaded from a mobile device to a
photo sharing service). Finally, before an image is displayed, each of
these steps is reversed until the pixels in each block have been
reconstructed.

\subsection{Why a New Recompression Strategy?}

\parab{Limitations of Traditional Approaches.} While photo storage services such as Flickr maintain a copy of the
original uploaded images, large-scale photo sharing services modify
the uploaded image in order to manage the scale of their storage
infrastructure. Specifically, Facebook (a) resizes images and (b)
recompresses them using a smaller quality parameter.

Resizing, while useful in managing storage, has its limits. Camera
resolution has been increasingly steadily over the last five years, as
have display resolutions, even on mobile devices. As a result, it is
likely that photo sharing services will increasingly face pressure to
serve high-resolution images in the near future, so photo sharing
services will need additional tools to manage photo storage. 

Recompressing an image by reducing JPEG's quality parameter (requantizing) is a
convenient knob for managing storage; for example, most cameras
generate high-quality images at quality parameter of 95, but Facebook reduces
the quality parameter on an uploaded image to \tld75. To achieve further storage saving, we have to apply the second quality parameter reduction. As we demonstrate experimentally in Section~\ref{eval}, two consecutive quality parameter reductions lead to unacceptable quality degradation.

In summary, while resizing and quality adjustments are currently used,
they are not a viable solution for producing additional storage
savings. Thus, in this paper we explore a completely different
approach for recompression, enabled by the unique setting of photo-sharing services.

\parab{New Opportunities in Photo-Sharing Services.} As opposed to traditional sender/receiver compression scheme where sender encodes the image and the receiver decodes it, the large-scale photo sharing services represent a new compression setting, with some special properties that offer opportunities for better compression.\footnote{We use encode/decode and compress/decompress interchangeably.}

\parae{Property 1: \emph{Collocated} Encoder/Decoder.}\label{the-collocated-encoderdecoder-setting} Instead of having two distinct sender/receiver entities where
the encoder and the decoder are in physically separate locations, the recompression setting in photo-sharing service includes both compression and decompression \emph{within the service}. In traditional distinct encoder/decoder setting data is typically encoded in one
of two ways. One is using a default codec (\emph{e.g.}, JPEG Standard)
that is present at the sender and receiver of the data and does not need
to be transmitted with it. The other is using a customized codec table
(\emph{e.g.}, JPEG Optimized) that is customized at the sender,
transmitted along with the data to the receiver, and then used to decode
the data. A customized codec table can typically represent the data more
compactly than a default table, but there is a tension between the size
of the codec table and the compactness of its representations. Larger
customized codec tables often lead to higher compression because they
can model the data more effectively. Yet, the customized codec table
must be kept small to ensure that the space savings obtained by the
richer encoding is not negated by having to transmit the table along
with the data.

\begin{figure}
\centering
\noindent\includegraphics[width=.9\columnwidth]{../figs/sender_receiver_and_self_sender-settings-crop.pdf}
\caption{Collocating the encoder and decoder enables the use of much larger and richer codecs.}
\label{fig:compression_settings}
\end{figure}

Figure \ref{fig:compression_settings} shows the
two ways data is encoded with a distinct encoder and decoder, and the
intuition behind why collocating the encoder and decoder enables the use
of richer customized codecs. In the collocated setting the encoder and
decoder are at the same location and thus the codec table used for
encoding the data can be decoupled from the data itself. This decoupling
removes the constraint on the size of codec tables: the codec tables can
be much larger than what is practical for individual files because they
are shared across many files and stored separately. As a result, this new design can potentially
reduce the storage footprint of a service beyond what standard
approaches can achieve.

\parae{Property 2: \emph{Large-Scale} Photo Storage.}\label{large-scale-storage} Despite the freedom to use large codec tables, the codec table
constitutes storage overhead that must be carefully managed. However,
the large-scale aspect of photo-sharing services helps in this regard: the same codec
overhead that would negate the additional storage reduction in a
small-scale case will become negligible for large-scale case as it will
be amortized across the entire storage (Figure
\ref{fig:saving_vs_photos}) because the codec tables are shared across
many photos. At small scales, our ROMP codec table (Section \ref{romp})
is much larger than a single image. If only one image was stored, the
footprint of the table and the image would be much bigger than the image
compressed with a normal, small JPEG table. In contrast, at large scale,
the size of the ROMP codec is negligible compared to the size of the
stored images, \emph{e.g.}, for ROMP, it needs to store 10,000 images to
make the codec negligible. Our evaluation in Section \ref{eval} shows
that these larger shared tables can compress photos better than
traditional customized tables, and have other benefits across the photo
stack.

\begin{figure}
\centering
\noindent\includegraphics[width=0.95\linewidth]{../exps/jpeg_vs_romp.eps}
\caption{Normalized storage size per photo of codec + image using JPEG Standard, JPEG Optimized, and ROMP for an increasing quantity of $2048\times1536$ photos. ROMP makes sense at the large scale it was designed for where the size of its larger codec is negligible compared to the storage saving it offers.}
\label{fig:saving_vs_photos}
\end{figure}

In summary, enabled by the collocating of encoder/decoder and the
large-scale setting, large codec tables can be used which would not be practical for traditional small-scale sender/receiver setting. In the following two subsections we describe: (a) ROMP, a lossless coding
technique that uses enhanced Huffman tables, and (b) L-ROMP, a perceptually
near-lossless coder that does not suffer from the significant quality
degradation inherent in re-quantization. Together, these techniques
can reduce photo storage requirements by 25\% or more, a significant
gain for large photo sharing services that store billions of images.

\subsection{ROMP: Lossless Coding using Enhanced Huffman Tables}
\label{sec:codec}\label{romp}

Our design, \sysname, exploits 
the decreasing cost of storing and managing large tables 
by designing \emph{context-sensitive coding tables} that result in
lossless compression. Recall that JPEG's Huffman tables are used to code symbols (information
about run-lengths and quantized values), 
based on the expected frequency of symbols' occurrence.
\sysname learns \emph{context-sensitive} Huffman tables by
learning the empirical probability of occurrence of these symbols from a large
corpus of images. This learning leverages the availability of such
corpora in a large-scale photo service. Concretely, \sysname uses below two
insights derived from properties of natural images to obtain context-sensitive Huffman tables.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{../exps/scatter/scatter_prob_zigzag2.pdf}
    %\shortentablecaptiona
    \shortenfigurecaption
    \caption{Probabilities of 3 Bit Coefficients at different positions.}
    %\shortentablecaptiona
    \label{fig:position_distribution}
    \vspace{-0.25in}
\end{figure}

\parab{Position-dependence.}
The empirical probability of
occurrence of a symbol can depend on its position in the 
zig-zag scan. 
That is, for a given symbol, its 
empirical probability of occurrence  at position $p_a$ along the 
zig-zag scan is likely
to be different from its empirical distribution at position $p_b$
(Figure~\ref{fig:position_distribution} illustrates this). 
For example, for natural images, it is known that
non-zero coefficients are increasingly unlikely at higher
frequencies~\cite{lam2000DCT}. Thus, if $p_b > p_a$ then a non-zero 
value will be less likely at $p_b$. For this reason, \sysname generates
different tables for different positions: i.e., position is one aspect
of the context used for encoding. Thus, the same symbol may be encoded
using different bit-patterns depending on the position where it occurs. 

\parab{Energy-dependence.}
The second insight is based on the observation that, relative to image
sizes predominantly in use today, an $8\times8$ block represents a
very small patch of the image.  To see this, imagine capturing the
same visual information (a photo of a person, say) with two cameras of
different resolutions, and then using JPEG encoding for both
images. Clearly $8\times8$ blocks in the higher resolution image
represent smaller regions of the field of view, and thus will tend to
be smoother.  This has two useful implications. First, information
within a block will tend to be smooth, with additional smoothness
expected for larger images. Smoother images are such that coefficients
at higher frequencies tend to be smaller. Second, because the same
region in the field of view comprises more blocks when larger images
(higher resolutions) are generated, it becomes more likely that
neighboring blocks will have similar characteristics.

We exploit these two ideas by creating tables such that the
probability of occurrence of a symbol at a given position can also
depend upon the \emph{energy} of other coefficients within the
block (\emph{intra-block} energy) and of neighboring blocks
(\emph{inter-block} energy). For a given \syma
that occurs at zigzag position $p$ of the $n$-th block, we use the
average of the observed coefficient sizes in a block as an estimate of intra-block 
energy: 
\begin{equation}
intra(n,p)=\frac{1}{p-1}\sum_{i=1}^{p-1}\frac{SIZE(b_n(i))}{max_{SIZE}(i)}
\label{formula:intra}
\end{equation}
where $b_{n}$ denotes the $n$-th block, and
$b_n(i)$ denotes the coefficient at position $i$, 
$SIZE(\cdot)$ denotes the bits required to represent the
amplitude of the coefficient, $max_{SIZE}(i)$ is the observed maximum
coefficient size for position $i$ of images in the training set.

Similarly, the inter-block energy value is estimated based on the 
average sizes of coefficients in nearby blocks: $F$
nearby zigzag positions in $B$ adjacent prior blocks (ROMP uses $F=5$ and $B=3$):
\vspace{-0.3cm}
\begin{equation}
inter(n,p)=\frac{1}{B\cdot F}\sum_{i=n-B}^{n-1}\sum_{j=p}^{p+F-1}\frac{SIZE(b_i(j))}{max_{SIZE}(j)}
\label{formula:inter}
\end{equation}

\begin{figure}[t]
%  \centering\epsfig{file=../pics/sysname.eps,  width=0.65\linewidth}
  \centering\includegraphics[width=0.65\linewidth]{../pics/sysname}
  %\shortentablecaptiona
  \caption{\sysname Encoding Architecture}
  %\shortentablecaptionb
 \label{fig:sysname}
 \vspace{-0.25in}
\end{figure}

\parab{Putting it all together.} Context in \sysname is defined by a triple $<p,i,e>$ to define context: zigzag position $p$, intra-block energy $i$ and inter-block energy $e$. Note that the statistical dependencies captured by this context information 
are well known in image coding and exploited by 
state of the art compression techniques, but to the best of our knowledge we are the first to take advantage of them for low latency JPEG transcoding (where complexity is minimized by using memory to store many, context-dependent Huffman tables). 

At a high-level, \sysname
works as follows (Figure~\ref{fig:sysname}). From a training set of images, \sysname learns a Huffman table for each unique context (i.e., for each unique combination of position, intra- and inter-block energy). For \syma that occurs in any image in the training set, \sysname first determines its context triple and then gathers it together with other \symas belonging to the same context. After gathering all the \symas for each context, \sysname can generate a table for this context based on the number of occurrences of each. \sysname pre-defines 20 different energy levels for both intra-energy and inter-energy, which leads to \tld$64\times20\times20=25600$ different contexts and Huffman tables to be learned.\footnote{These tables take up  less than 16MBs of the memory, a negligible memory usage increment for modern machines.} These tables are quite different, which allows \sysname to achieve better compression over standard JPEG. When an image is uploaded, \sysname decodes the JPEG image, computes the corresponding triple $<p,i,e>$, the then uses the learned Huffman tables to re-code the image. Before delivering an image to a client, \sysname reverses its context-sensitive entropy code, then applies the default JPEG entropy code.

\subsection{L-ROMP: A Gracefully Lossy Coder}
\label{sec:codec_lossy}

\sysname's entropy coder is lossless with respect to the uploaded
JPEG. In this section, we describe \lossyname, which introduces a controlled, perceptually insignificant, amount of loss
(or \emph{distortion}) in uploaded images, as a way of achieving
further savings in photo storage. 

As discussed previously, users upload high quality JPEG images and  many photo sharing services, e.g., Facebook, change the JPEG quality  parameter to a lower level in order to ensure predictable storage usage, a step that introduces additional distortion~\cite{coulombe2010transcoding}. Figure~\ref{fig:better_transcoding} quantifies the dramatic increase in distortion caused by re-quantization, compared to quantizing the original raw image directly to the target quality parameter, showing rate-distortion performance with two different objective quality metrics: PSNR and MS-SSIM. The ``Re-quantize (raw)'' curve is obtained by reducing the quality parameter when compressing the original raw images, while the ``Re-quantize (JPEG)'' curve is obtained by re-quantizing a high-quality JPEG image derived from the same set of raw images. The former curve represents much more graceful degradation. By contrast, re-quantization introduces much more distortion for the same size reduction. This happens because the latter suffers from cumulative errors due to two consecutive re-quantizations. 


\begin{figure}[t]
  \centering
    \includegraphics[width=1.05\linewidth]{../pics/plot_msssim.eps}
\vspace{-0.5cm}
  \caption{Rate/distortion performance of \lossyname, compared to re-quantization from raw image and from JPEG image using Tecnick images of 1200$\times$1200. \textbf{(a)}: Using PSNR as the quality metric, and showing performance on JPEG images of four quality parameters (70,80,86,90). \textbf{(b)}: Using MS-SSIM metric, and focusing on JPEG images of quality paramter of 75; ``o'' marks the perceptually lossless setting of \lossyname.}
 \label{fig:better_transcoding}
\vspace{-0.5cm} 
\end{figure}

\lossyname avoids re-quantizing coefficients, but
introduces distortion by carefully setting \emph{some} non-zero
(quantized) coefficients to zero, a specific instance of a general
idea called thresholding~\cite{thresholding}. The intuition behind thresholding is
that, by setting a well-chosen non-zero coefficient to zero, it is
possible to increase the number of consecutive zero-valued
coefficients in the sequence of coefficients along the zig-zag scan. 
This in general helps 
reduce size as it replaces two separate runs of zeros together 
and a non-zero coefficient value, by a single run of zeros. Optimization of coefficient thresholding has been considered from a 
rate-distortion perspective in the literature~\cite{ortega1998rate,thresholding}, we are not
aware of it being explored as an alternative to re-quantization in
large photo sharing services.
Here we use a simplified version where only coefficients of size equal to 1 (i.e., $1$ or
$-1$) can be removed. This means that the distortion increase for any coefficient 
being removed will be the same.\footnote{Note that the actual MSE will be different if 
two coefficients have same value $1$, but different frequency weights in the quantization 
matrix. However, by ignoring this difference we take into account the different perceptual 
weighting given to each frequency and obtain better perceptual quality.} Thus, we only need to decide if for a given 
coefficient the bit-rate savings are sufficient to remove it. We make the decision by introducing a \emph{rate threshold} and only thresholding a coefficient if the bits saving by doing so would exceed this threshold.

However, setting too many coefficients to zero within a block can
introduce local artifacts (e.g., blocking). Thus, \lossyname uses 
a \emph{perceptual threshold} $T_p$ that limits 
the percentage of non-zero  
coefficients that will be set to zero.
By doing this \lossyname can guarantee that the block-wise SSIM with respect to the original 
JPEG is always higher than $1-\frac{T_p}{2-T_p}$. 
For example, if we use $T_p=0.1$ (i.e., we can threshold at most 10\% of the non-zero coefficients), then block-wise SSIM metric is guaranteed to be higher than 0.947. 
The proof of such bound is based on results from~\cite{ssim_distortion} and is omitted for brevity.

In Figure~\ref{fig:better_transcoding} (a), we observe that \lossyname degrades PSNR more gracefully than simply re-quantizing. We see that with conservative thresholds, \lossyname's curve is actually higher than re-quantizing from the raw image curve, illustrating the efficiency of \lossyname's trading distortion for bits-saving. \lossyname performs equally well on MS-SSIM metric (plot (b)). To achieve perceptually lossless compression, we also conducted a subjective evaluation, by developing a comparison tool that can choose thresholds and shows the image at the chosen setting as well as size reduction. We find that using rate threshold of 2.0 and perceptual threshold of 0.4 provides maximum bits-saving without noticeable quality distortion (``o'' of Figure~\ref{fig:better_transcoding} (b)). We use these parameters for L-ROMP.

Finally, \lossyname can be easily introduced into \sysname's
pipeline: before applying the
context-sensitive entropy coding, 
\lossyname's thresholding can be
applied to each block (Figure~\ref{fig:sysname}). No changes are
required to \sysname's entropy coder.


==> tbl_cache_effects.tex <==
\newcommand{\twor}[1]{\multirow{2}{*}{#1}}
\begin{table}[t]
\begin{tabular}{l rrr}
\toprule[1.5pt]
\centering
                        & \textbf{\sysname} & \textbf{\lossyname} & \textbf{\aggrename} \\
Compression             &     13\% &       26\% &       ??\% \\
\midrule

Effective Cache Size    &    1.15$\times$ &      1.35$\times$ &      1.54$\times$ \\[0.5ex]
Hit Ratio Increase      &&&\\
\quad Edge Cache        &    1.1\% &      2.5\% &      3.9\% \\
\quad Origin Cache      &    1.6\% &      3.8\% &      5.9\% \\[0.5ex]

Fewer Requests          & \twor{4.9\%} & \twor{11.4\%} & \twor{17.1\%} \\
To The Backend          &&&\\[0.5ex]
%Fewer Bytes to Backend & 17.3\%   & 33.1\%     & 46.1\%     \\[0.5ex]

Fewer Bytes Sent        & \twor{15.2\%} & \twor{30.5\%} & \twor{41.0\%} \\
To The Edge             &&&\\[0.5ex]

Reduction in            & \twor{0.0\%} & \twor{15.5\%} & \twor{25.0\%} \\
External Bandwidth      &&&\\%[0.5ex]
\bottomrule[1.5pt]
\end{tabular}
\caption{Estimated collateral benefits from deploying \sysname in the Facebook photo caching stack.}
%   caching stack based on compression for larger photos.  The storage
%   reduction from \sysname and \lossyname is calculated as a percentage of
%   the logical size of photos stored in Facebook's Haystack~\cite{haystack} and f4~\cite{f4}
%   systems.  The effect of caching smaller objects through increased
%   hit ratio and decreased cache-fill bandwidth or backend requests, or
%   the amount of current cache could be shrunk and achieve the same hit
%  ratio is shown for the edge and origin caches.}
\label{tbl:cache_effects}
\end{table}


==> tbl_cache_effects_aromp.tex <==
%\newcommand{\twor}[1]{\multirow{2}{*}{#1}}
\begin{table}[t]
\centering
\begin{tabular}{l r}
\toprule[1.5pt]
\centering
%                        & \textbf{\sysname} & \textbf{\lossyname} & \textbf{\aggrename} \\
Compression             &    34\% \\
\midrule

%Effective Cache Size    &    1.54$\times$ \\[0.5ex]
%Hit Ratio Increase      &\\
%\quad Edge Cache        &    3.9\% \\
%\quad Origin Cache      &    5.9\% \\[0.5ex]

Fewer Requests          & \twor{16.4\%} \\
To The Backend          &\\[0.5ex]
%Fewer Bytes to Backend & 17.3\%   & 33.1\%     & 46.1\%     \\[0.5ex]

Fewer Bytes Sent        & \twor{38.3\%} \\
To The Edge             &\\[0.5ex]

Reduction in            & \twor{22.0\%} \\
External Bandwidth      &\\%[0.5ex]
\bottomrule[1.5pt]
\end{tabular}
\caption{Estimated collateral benefits from deploying \aggrename in the Facebook photo caching stack.}
%   caching stack based on compression for larger photos.  The storage
%   reduction from \sysname and \lossyname is calculated as a percentage of
%   the logical size of photos stored in Facebook's Haystack~\cite{haystack} and f4~\cite{f4}
%   systems.  The effect of caching smaller objects through increased
%   hit ratio and decreased cache-fill bandwidth or backend requests, or
%   the amount of current cache could be shrunk and achieve the same hit
%  ratio is shown for the edge and origin caches.}
\label{table:aromp}
\end{table}


==> tbl_cache_effects_without_aromp.tex <==
\newcommand{\twor}[1]{\multirow{2}{*}{#1}}
\begin{table}[t]
\centering
\begin{tabular}{l rr}
\toprule[1.5pt]
\centering
                        & \textbf{\sysname} & \textbf{\lossyname}\\
Compression             &     13\% &       26\%\\
\midrule

Effective Cache Size    &    1.15$\times$ &      1.35$\times$\\[0.5ex]
Hit Ratio Increase      &&\\
\quad Edge Cache        &    1.1\% &      2.5\%\\
\quad Origin Cache      &    1.6\% &      3.8\%\\[0.5ex]

Fewer Requests          & \twor{4.9\%} & \twor{11.4\%}\\
To The Backend          &&\\[0.5ex]
%Fewer Bytes to Backend & 17.3\%   & 33.1\%     & 46.1\%     \\[0.5ex]

Fewer Bytes Sent        & \twor{15.2\%} & \twor{30.5\%}\\
To The Edge             &&\\[0.5ex]

Reduction in            & \twor{0.0\%} & \twor{15.5\%}\\
External Bandwidth      &&\\%[0.5ex]
\bottomrule[1.5pt]
\end{tabular}
\caption{Estimated collateral benefits from deploying \sysname in the Facebook photo caching stack.}
%   caching stack based on compression for larger photos.  The storage
%   reduction from \sysname and \lossyname is calculated as a percentage of
%   the logical size of photos stored in Facebook's Haystack~\cite{haystack} and f4~\cite{f4}
%   systems.  The effect of caching smaller objects through increased
%   hit ratio and decreased cache-fill bandwidth or backend requests, or
%   the amount of current cache could be shrunk and achieve the same hit
%  ratio is shown for the edge and origin caches.}
\label{tbl:cache_effects}
\end{table}


==> tex_for_2x3_subfigures.tex <==
% this is a subfigure arrangement with mini-page
\begin{figure*}[t]
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{A}
  \label{ex0}
\end{subfigure}\\
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{B}
  \label{ex3}
\end{subfigure}
\caption{caption for Fig 11a, 11b}
\end{minipage}
%second column
\begin{minipage}[t]{0.34\textwidth}
\centering
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{A}
  \label{ex0}
\end{subfigure}\\
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{B}
  \label{ex3}
\end{subfigure}
\caption{caption for Fig 12a, 12b}
\end{minipage}
%third column
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{A}
  \label{ex0}
\end{subfigure}\\
\begin{subfigure}[b]{1\linewidth}
  \centering
  \includegraphics[scale=0.55]{../exps/comp_vs_quality/comp_vs_enc_1152_final.pdf}
  \caption{B}
  \label{ex3}
\end{subfigure}
\caption{caption for Fig 13a, 13b}
\end{minipage}
\caption*{One big caption for all}
\vspace{-0.15in}
\end{figure*}

